Sampling and Representation Complexity of Revenue Maximization

We consider (approximate) revenue maximization in auctions where the distribution on input valuations is given via "black box" access to samples from the distribution. We observe that the number of samples required -- the sample complexity -- is tightly related to the representation complexity of an approximately revenue-maximizing auction. Our main results are upper bounds and an exponential lower bound on these complexities.

==> Zbackup_nets_Li.tex <==
\section{Nets and Sample Complexity}
\label{sec:nets}


\begin{note}(Shaddin)
 Should we move to $[1,H]$ valuations for these positive results? I tried, and its a bit of a mess. Made me wonder if doing so is worth it, given that the additive results in $[0,1]$ are only stronger (i.e. they imply multiplicative approximations for $[1,H]$ valuations in $\poly(H)$ time). I left partial progress in nets.multiplicative.tex.

A resonable strategy would be to have positive results in $[0,1]$, and negative results in $[1,H]$.
\end{note}


\begin{definition}
  Let $\N$ and $\M$ be two families of menus, and $\V \sse [0,1]^m$ a family of valuations. We say $\N$ is a \emph{one-sided $\epsilon$-net} of $\M$ with respect to $\V$ if for every $M \in \M$ there is $N \in \N$ such that for all $v \in \V$ \begin{align}\label{eq:epsnet}\Rev(N,v) \geq \Rev(M,v) - \epsilon.\end{align} We say the net is \emph{effective} if there is an algorithm  which takes as input $M \in \M$ and outputs $N \in \N$ with $|N| \leq |M|$ satisfying \eqref{eq:epsnet} in time $\poly(|M|,m,\frac{1}{\eps})$.  
\end{definition}



\begin{theorem}\label{thm:nets1}
  If $\N$ is a finite one-sided $\epsilon$-net of $\M_\infty$ with respect to $\V \sse [0,1]^m$, then there is an $\eps$-approximation algorithm for the pricing problem in the black box model which makes $n=\poly(m,\log |\N|, \frac{1}{\eps})$ queries. Moreover, if the net is effective, then the algorithm runs in time polynomial in $n$.
\end{theorem}
\begin{proof}
  
\end{proof}

\begin{theorem}\label{thm:nets2}
  If $\N$ is a finite one-sided $\epsilon$-net of $\M$ with respect to $\V \sse [0,1]^m$, then there is an algorithm for the pricing problem in the black box model which makes $n=\poly(m,\log |\N|, \frac{1}{\eps})$ queries, and outputs $N \in \N$ such that $\Rev(N,\D) \geq \Rev(\M,\D) - \eps$.
\end{theorem}
\begin{proof}
  
\end{proof}


Our main technique for constructing $\epsilon$-nets of menus is through constructing an $\eps$-net of the set of lotteries.

\begin{definition}
  A family $\L \sse \Delta_m$ of lotteries is a (two-sided) $\epsilon$-net of $\Delta_m$ with respect to $\V$ if for every $x \in \Delta_m$ there is $y \in \L$ such that the following holds for all $v \in \V$ \begin{align}\label{eq:epsnet_val} |v \cdot x - v\cdot y| \leq  \eps\end{align} Moreover, we say the net is \emph{effective} if there is an algorithm which takes as input $x \in \Delta_m$ and outputs $y \in \L$ satisfying \eqref{eq:epsnet_val} in time $\poly(m,\frac{1}{\eps})$
\end{definition}

\begin{lemma}\label{lem:lottery_to_menu_net1}
  If $\L$ is an $\epsilon^2$-net of $\Delta_m$ with respect to $\V \sse [0,1]^m$, and $\M$ is a family of menus, then there is a one-sided $6\eps$-net  $\N$ of $\M$ with respect to $\V$ witn $|\N| \leq \frac{1}{\eps^2}^{|\L|}$. Moreover, if $\L$ is effective, then so is $\N$. 
\end{lemma}
\begin{proof}

For each $M \in \M$, include in $\N$ an approximation $\tilde{M}$ of $M$, defined as follows. For every $(x,p)$ in $M$, include in $\tilde{M}$ an entry  $(\tilde{x},\tilde{p})$ satisfying:
\begin{itemize}
\item $\tilde{x} \in \L$ and $|v \cdot x - v \cdot \tilde{x} | \leq \eps^2$ for every $v \in \V$ 
\item Let $t \eps^2$ be the result of rounding down $p$ to the nearest integer multiple of $\eps^2$, and let $\tilde{p}= t (\eps^2 - \eps^3)) $
\end{itemize}

We now claim that $\Rev(M, v) - \Rev(\tilde{M},v) \leq 6 \eps$ for every $v \in \V$. Intuitively,  the mapping $(x,p) \to (\tilde{x},\tilde{p})$ described above changes a player's value for allocation $x$ by at most $\eps^2$, and reduces the price $p$ by a quantity between $\eps^2$ and $ \eps+\eps^2$ which increases as $p$ increases. This increasing discount for pricy lotteries makes them comparatively more attractive, limiting the decrease in revenue. Formally, for $(x,p) \in M$, we can bound the change of utility  $(v \cdot \tilde{x} - \tilde{p}) - (v \cdot x - p)$ as follows.
\begin{align*}
  p\eps + 2 \eps^2 \geq  \floor{p/\eps^2} \eps^3 + 2\eps^2  \geq (p-\tilde{p}) - (v \cdot x - v\cdot \tilde{x})  
\geq \floor{p/\eps^2} \eps^3 - \eps^2 \geq p \eps - 2 \eps^2
\end{align*}

Now assume that a buyer $v$ buys lottery $(x,p) \in M$, and $(\tilde{y},\tilde{q}) \in M'$. 
%
%
\begin{align*}
v \cdot y - q  &\leq v \cdot x - p \\ 
v \cdot \tilde{y} - \tilde{q}  &\geq v \cdot \tilde{x} - \tilde{p} \\
q\eps + 2 \eps^2 \geq (v \cdot \tilde{y} - \tilde{q}) - (v \cdot y - q)&\geq (v \cdot \tilde{x} - \tilde{p}) - ( v \cdot x - p) \geq p\eps - 2 \eps^2  \\
q\geq p - 4 \eps \\
\end{align*}

Since $\tilde{q} \geq q - \eps - \eps^2$, we conclude that $\tilde{q} \geq p - 6 \eps$, establishing that $\N$ is a one-sided $\epsilon$-net of $\M$. Moreover, since $\L$ is effective, the mapping $M \to \tilde{M}$ is proof that $\N$ is effective.
\end{proof}


\begin{lemma}\label{lem:lottery_to_menu_net2}
  If $\L$ is an $\epsilon^2$-net of $\Delta_m$ with respect to $\V \sse [0,1]^m$, then there is a one-sided $6\eps$-net  $\N \sse \M_k$ of  $\M_k$ with respect to $\V$ with $|\N| \leq ( \frac{|\L|}{\eps^2})^k$. Moreover, if $\L$ is effective, then so is $\N$. 
\end{lemma}
\begin{proof}
The net is $\N$ is constructed as in the proof of Lemma \ref{lem:lottery_to_menu_net1}. When $\M=\M_k$ it is easy to see that $|\N| \leq ( \frac{|\L|}{\eps^2})^k$.
\end{proof}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pricing"
%%% End: 


==> Zbackup_small_Li.tex <==
\section{The Complexity of Small Menus}
\label{sec:small}

In this section, we consider the mechanism design problem when  an auctioneer looking to design a near-optimal ``small'' menu. This may be for one of two reasons: either the auctioneer has reason to believe that there exists a near optimal menu which happens to be small, or else he is constrained by practical considerations to such menus. Specifically, we consider the \emph{$k$-menu pricing problem}, in which the auctioneer must choose a $k$-menu maximizing expected revenue over a distribution $\D$ of valuations given by a black box. In this section,  our only assumption on $\D$ is that it is supported on $\V = [0,1]^m$.


\subsection{The Sample Complexity of Designing Small Menus}

We begin by examining the sampling complexity of the $k$-menu pricing problem. We apply the ideas of Section \ref{sec:nets} to prove that it suffices to sample $\D$ a small number of times. Specifically, when valuations are bounded,  a random sample of $n=\poly(m,k)$ valuations from $\D$ suffices for identifying a near optimal $k$-menu.% This can be viewed as a sample complexity result for the set of small menus, in that it bounds the number of samples needed for the empirical distribution approximate the revenue of the original distribution $\D$ on every such menu. 

\begin{theorem}\label{thm:sample_small}
When $\V=[0,1]^m$, there is an algorithm for the single-buyer mechanism design problem  in the black box model which makes $n=\poly(m,k, \frac{1}{\eps})$ queries, and outputs a $k$-menu $M$ such that $\Rev(M,\D) \geq \Rev_k(\D) - \eps$.
\end{theorem}
 We note that, when a near-optimal small $k$-menu exists, the above theorem yields an $\epsilon$-approximation algorithm for the pricing problem. However this result is information theoretic, and does not provide an efficient algorithm.  
%
The proof of the above theorem follows by combining the proposition below with Lemma \ref{lem:lottery_to_menu_net2} and Theorem \ref{thm:nets2}.
\begin{proposition}\label{prop:lottery_net}
  For every $\eps > 0$, there is an effective $\epsilon$-net $\L(\epsilon) \sse \Delta_m$ of $\Delta_m$ with respect to $[0,1]^m$. Moreover,  $|\L(\epsilon)| \leq \left(\frac{1}{\epsilon}\right)^{\tilde{O}(m)}$.
\end{proposition}
\begin{proof}
  Let $\L(\epsilon)$ be the set of all lotteries $x \in \Delta_m$ in which each entry $x_i$ is an integer multiple of $\frac{\eps}{m}$. Evidently, each $x_i$ may take on at most $\frac{m}{\eps}$ possible values, so $|\L(\epsilon)| \leq \left(\frac{m}{\eps}\right)^m$.

Consider $x \in \Delta_m$. To complete the proof, it suffices to exhibit $x' \in \Psi$ such that $|v \cdot x - v \cdot x'| \leq \epsilon$ for every $v \in [0,1]^m$. Let $x'$ be the result of rounding down each entry of $x$ to the nearest multiple of $\frac{\epsilon}{m}$. Observe that $|v_i x_i - v_i x'_i| \leq \frac{\eps}{m}$. Therefore $|v \cdot x - v \cdot x'| \leq \eps$, as needed.
\end{proof}



\subsection{The Computational Complexity of Designing Small Menus}
%We now consider the task of a seller looking to design an optimal ``small'' menu. Even in settings in which revenue can grow linearly in the size of a menu (Theorem \ref{thm:menu_complexity}), a seller may be constrained to small menus due to practical considerations. As an example, consider a restauranteur looking to design a new dinner menu. As no customer can be reasonably expected to select from thousands of menu items, the restaurant may place a reasonable bound $k$ on the number of meals on offer. 

----------- CONTINUE HERE ------------

In this section, we examine the computational complexity of the algorithmic task associated with Theorem \ref{thm:sample_small}.
Let $X$ be an explicitly given distribution $\{v_1, \cdots, v_n\} \sse \V$. We define the optimization problem $MAXREV(X,k)$ as that of computing the revenue maximizing menu of size at most $k$ for a buyer drawn uniformly from $X$. 

\begin{thm}\label{thm:maxrev_nphard}
$MAXREV(X, k)$ in NP-hard to approximate to within any factor better than $\frac{e}{e-1}$, even for valuations $\V= \set{0,1}^m$.
\end{thm}
\begin{proof}
Let $n=|X|$. As all valuations are $\{0,1\}$ vectors, each $v_i \in \X$ corresponds to a subset $S_i = \{ i
\in [m] : v_i = 1\}$ of the items $[m]$. 

We begin by observing that there is an optimal $k$-menu which is an item pricing menu. When $k\geq m$ this is clear, as the seller can do no better than pricing every item at $1$. Now assume $k <m$, and let $M = \{(x_1,p_1), \ldots (x_k,p_k)
\}$ be an optimal lottery pricing $k$-menu. Let $X_j \subseteq [n]$ denote
the set of valuations $v_i$ that chooses lottery $(x_j, p_j)$. 
Observe that the
sets $X_1,\ldots,X_k$ are disjoint, and the revenue is $\sum_{j=1}^k
\frac{|X_j|}{n} p_j$.
Moreover, by individual
rationality, 
every $v_i \in X_j$ satisfies $v_i \cdot x_j \geq p_j$. 
In other words, an item drawn at random
from lottery $x_j$ ``hits'' $S_i$ with probability at least $p_j$. 

Now, consider drawing $k$ items $j_1,\ldots,j_k$ independently, 
one from each of the lotteries
$x_1,\ldots,x_k$. 
For $x_1$, in expectation, the number of valuations ``hit'' by $j_1$ is at least
$|X_1| p_1$. 
Therefore, there is a set of $k$ items that collectively hit at least
$\sum_{j=1}^k |X_j| p_j$ valuations. Setting a price of $1$ for each of these
items gathers that much in revenue. 



To show NP-hardness, we reduce from the NP-hard problem max cover, which is known to be hard to approximate by any factor better than $\frac{e}{e-1}$. For convenience, we use the ``hitting set'' formulation of max cover. The input to this problem is a family $\S=\set{S_1,\ldots,S_n}$ of subsets of $[m]$, and an integer $k$, and the outputs is a ``hitting set'' $M \sse [m]$ of size at most $k$ maximizing the number of sets $S \in \S$ with which $M$ has a non-empty intersection.   Given an instance $(\S,k)$ of max cover, we construct an instance $(X,k)$ of $MAXREV$ by letting $X = \set{v_S : S \in \S}$, where $v_S$ denotes the indicator vectof of $S \sse [m]$. It is not hard to see that the revenue of the optimal $k$-lottery equals the number of sets in $\S$ hit by the optimal hitting set of size at most $k$. Since this reduction is approximation preserving, hardness of approximation follows.
\end{proof}

\begin{thm}
There is a polynomial-time $(1-1/e)$-approximation algorithm for $MAXREV$ when $\V\sse \set{0,1}^m$.
\end{thm}
\begin{proof}
  The reduction from the max cover problem used in the proof of Theorem \ref{thm:maxrev_nphard} is reversible. Therefore, using the $(1-1/e)$ approximation for max cover yields the same guarantee for $MAXREV$.
\end{proof}


\subsubsection{Open Question}

\paragraph{Open Question:} What is the best approximation possible for MAXREV when the valuations $\V \sse [0,1]^n$ are arbitrary yet bounded?

\paragraph{Conjecture:} We conjecture that there is no constant approximation algorithm, even when $k=1$. In other words, we conjecture that it is hard to find the best single lottery for an explicitly given list of unit-demand valuations! We make this conjecture because of an apparent similarity between this problem and the problem of finding a ``maximum satisfying linear subsystem.'' To see this connection, we phrase $MAXREV(.,1)$ slightly differently.

\paragraph{Alternative Formulation of $MAXREV$ for $k=1$:} Given a matrix $V$ with nonnegative entries, where $v_i$ is the i'th row of V, find a probability vector $x$ and real number $p$ maximizing $p | V x \geq p|$, where $| Vx \geq p|$ is short-hand for the number of the satisfied equations in the system $V x \geq p$. Given an appropriate guess for $p$, a moment's thought reveals that this problem reduces to finding a nonnegative and non-zero vector x satisfying as many as possible of the inequalities $V' x \geq 0$, where $V'_{ij} = V_{ij} - p$. This appears closely related to the ``maximum satisfying linear subsystem'' problem, though we have not yet succeeded in proving hardness.

\paragraph{Summary of Progress so Far:} We succeeded in proving that maximizing  $|V x \geq p|$ for a \emph{given} price $p$ is as hard to approximate as independent set. However, this does not rule out constant approximation algorithms for $MAXREV(.,1)$, since the problem may be easy to approximate for some $p'$ which is slightly smaller (within a constant factor) than the optimal price. Moreover, an $O(\log n)$ approximation algorithm for $MAXREV(.,1)$ is relatively straightforward by  a bucketing argument, followed by applying the constant approximation algorithm for MAXREV with $\set{0,1}$-valuations. Other than that, we appear to be somewhat stuck, though reductions from unique games or label cover appear to be promising approaches for showing hardness.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pricing"
%%% End: 


==> app-classes.tex <==
\section{Proofs from Section \ref{sec:classes}}
\label{app:classes}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pricing"
%%% End: 


==> app-computational.tex <==
\section{Proofs from Section \ref{sec:computational}}
\label{app:computational}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pricing"
%%% End: 


==> app-description.tex <==
\section{Proofs from Section \ref{sec:description}}
\label{app:description}
\begin{proposition}[continues=prop:logH]
There exists a menu $M$ with $m$ entries satisfying $Rev(M,\D) \ge \frac{1}{O(\log H)}  Rev(\D)$. Moreover, there is a polynomial time algorithm which makes $\poly(H)$ samples and outputs  such a menu with high probability.
\end{proposition}
\begin{proof}
Let $M^p$ denote the $m$-entry menu which offers every item for a price of $p$; i.e. $M^p = \{(e_i, p) : i \in \set{1,\ldots,m}\}$, where $e_i$ is the $i$'th standard basis vector. One of the $\log H$ menus $M^1, M^2, M^4, \ldots, M^H$ is guaranteed to extract a $1/2\log H$ fraction expected maximum value for an item $\Ex_{v \sim D} \max_i v_i$, which in turn is an upper bound on the maximum revenue. 

To make this algorithmic, observe that the revenue of each of $M^1, M^2, M^4, \ldots, M^H$ is a random variable between $0$ and $H$.  The algorithm is the obvious one: take $n=\omega(H^2 \log \log H)$ samples from $\D$, and return the menu from $M^1, M^2, M^4, \ldots, M^H$  with the greatest expected revenue on the sample. By applying the Hoeffding bound and the union bound, our estimate for the revenue of each menu $M^p$ is within an additive error of $1/2$ with high probability. Since $\Rev(\D) \geq 1$, the chosen menu satisfies the claimed bound.
\end{proof}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pricing"
%%% End: 


==> app-nets.tex <==
\section{Proofs from Section \ref{sec:covers}}
\label{app:covers}


\begin{lemma}\thmcontinues{lem:lottery_to_menu_cover}
Fix $\epsilon >0$ and $k \in \NN \union \set{\infty}$. 
  If $\L$ is an $\frac{\epsilon^2}{\log H}$-cover of $\Delta_m$ with respect to $\V \sse
  [1,H]^m$, then there is a one-sided $8\eps$-cover
  $\N$ of $\M_k$ with respect to $\V$ with $|\N| \leq  \min\left\{\left(\frac{\log H}{\eps}\right)^{2|\L|},  \left(\frac{ \log^2 H |\L|}{\eps^2}\right)^k \right\}$ and $\N \sse \M_{|\L|}$. 
%  If $\L$ succinct then so is $\N$, and if $\L$ is effective then so is $\N$.
Moreover, if $\L$ is effective then so is $\N$.
\end{lemma}

\begin{proof}
Denote $\sigma = \frac{\epsilon^2}{\log H}$. We define for every (non-zero) allocation/price pair $(x,p)$ a rounded version $(\tilde{x},\tilde{p}) = r(x,p)$, as follows:
\begin{itemize}
\item Let $ p' = e^{t\sigma}$ be the result of rounding $p$ down to the nearest integer power of $e^\sigma$. Note that $t(p) \in \set{0,1,\ldots,\left\lfloor{\frac{\log H}{\sigma}}\right\rfloor}$
\item Let $x' \in \L$ satisfy $e^{-\sigma} v \cdot x - \sigma \leq v \cdot x' \leq e^\sigma v \cdot x + \sigma$  for every $v \in \V$. (Equation \eqref{eq:epscover_lottery})
\item Define the ``bonus'' multiplier $b=b(p)=  e^{t \sigma^2/\eps }$. Note that $b(p) \in [1, e^{\eps}]$ is nondecreasing in $p$.
\item Define the ``discount'' $d=d(p) = t \frac{\sigma^2}{\eps}$. Note that $d(p) \in [0,\eps]$.
\item Let $\tilde{p} = e^{- \eps}  \cdot p' / b - d$, and $\tilde{x} = e^{-\eps} \cdot b \cdot x'$. 
%\item Let $\tilde{x} =  e^{t  \sigma^2 / \eps - \eps} x'$. Note that $ e^{-\eps} x' \leq \tilde{x} \leq x'$ component-wise.
\end{itemize}
We naturally extend this definition to menus. For each menu $M$, we let $\tilde{M} = \set{r(x,p): (x,p) \in M}$. Finally, we define our net $\N$ as the set of all rounded menus from $\M$, i.e. $\N = \set{\tilde{M} : M \in \M}$. 
 %It is easy to see that $\N$ is succinct when $\L$ is succinct, and $\N$ is effective when $\L$ is effective.
By examining the map $M \to \tilde{M}$, it is easy to see that $\N$ is effective when $\L$ is effective.

Note that rounded allocation/price pairs $(\tilde{x},\tilde{p})$ are in one to one correspondance with $\L \cross \set{0,1,\ldots,\left\lfloor{\frac{\log^2 H}{\eps^2}}\right\rfloor}$. Since, without loss of generality, every lottery appears at most once in any menu $N \in \N$, we have that $N \sse \M_{|\L|}$ and  $|\N| \leq \left(\frac{\log H}{\eps}\right)^{2|\L|}$.  Moreover, since every $N \in \N$ has at most $k$ entries, each of which is a rounded allocation/price pair, we have that $|\N| \leq \left(\frac{ \log^2 H |\L|}{\eps^2}\right)^k$.


We now claim that $\Rev(M, v) \geq e^{-8\eps} \Rev(\tilde{M},v)$ for every $v \in \V$.  Intuitively,  the mapping $r: (x,p) \to  (\tilde{x},\tilde{p})$ can be thought of as the composition of two mappings: $(x,p) \to (x',p')$ and $(x',p') \to (\tilde{x},\tilde{p})$. The former introduces error into each of $v \cdot x$ and $p$, which may have the undesirable consequence of changing a player's choice and thus reducing the auctioneer's
 revenue on $v$. The purpose of the latter mapping is to fix this by providing a bonus/discount for pricy lotteries in order to make them comparatively more attractive.

Formally, assume for a contradiction that $\Rev(M, v) < e^{-8\eps} \Rev(\tilde{M},v)$ for some $v \in \V$. Let $(x,p)$ be the chosen allocation/price pair from menu $M$, and $(\tilde{y},\tilde{q}) = r(y,q)$ be the chosen pair from menu $\tilde{M}$.  Denoting $(\tilde{x},\tilde{p}) = r(x,p)$, it follows that

\begin{align}
(v \cdot x - v \cdot y)  - (p - q) &\geq 0  & &\mbox{(By the choice of $(x,p)$ from $M$)} \label{eq:pq}\\
(v \cdot \tilde{x} - v \cdot \tilde{y})  - (\tilde{p} - \tilde{q}) &\leq 0 & &\mbox{(By the choice of $(\tilde{y},\tilde{q})$ from $\tilde{M}$)} \label{eq:pqtilde}
\end{align}

\noindent Moreover, $p$ is significantly larger than $q$.

\begin{align}\label{eq:bonuspq}
p &> e^{8 \eps} \tilde{q} \notag &&\mbox{(By assumption)} \\
&= e^{7 \eps}  q' / b(q) - d(q) \notag &&\mbox{(By definition of $r(.)$)} \\ 
&\geq e^{6 \eps} q'  - \eps  \notag  &&\mbox{(Since $b(q) \leq e^\eps$ and $d(q) \leq \eps$)} \\
&\geq e^{6 \eps - \sigma} q - \eps \notag &&\mbox{(Since $q' \geq e^{-\sigma} q$, by definition)}  \\ 
& \geq e^{5 \eps} q - \eps \notag &&\mbox{(Since $\sigma \leq \eps$)}  \\
& \geq e^{4 \eps} q.  & & \mbox{(Since prices are at least 1 (see Section \ref{sec:prelim}))}
\end{align}


Inequality \eqref{eq:bonuspq} and the definition of $r(.)$ imply that $t(p) - t(q) \geq  \frac{4 \eps}{\delta}$, and therefore that $\frac{b(p)}{b(q)} \geq e^{\frac{4 \eps}{\delta} \frac{\delta^2}{\eps}}= e^{4\sigma} $ and $d(p) - d(q) \geq \frac{4 \eps}{\delta} \frac{\delta^2}{\eps} = 4 \sigma$; i.e. the larger price is given a substantially larger bonus and discount. Using this fact, we reach a contradiction with \eqref{eq:pq} and \eqref{eq:pqtilde}, completing the proof.


% \begin{claim}
%   Assume $(x,p)$ and $(y,q)$ are such that $q < p - \eps$. It is the case that $\tilde{p} - \tilde{q} \leq e^{-\eps} (p- q)$.
% \end{claim}
% \begin{proof}
  \begin{align}
    \tilde{p} - \tilde{q} &= e^{- \eps} ( p' / b(p) -  q' / b(q)) - (d(p) - d(q) &  \mbox{(By definition of  $r(.)$)} \notag\ \\
 & \leq e^{- \eps} (  p / b(p) - q e^{-\sigma} / b(q)     )  - (d(p) - d(q)) & \mbox{(Since $p' \leq p$ and $q' \geq e^{-\sigma} q$)} \notag\\
&\leq e^{- \eps} (  p / b(p) - q  / b(p)  ) - 4 \sigma & \mbox{(Since $b(p) \geq e^\sigma b(q)$ and $d(p) - d(q) \geq 4 \sigma$)} \notag\\
&\leq e^{- \eps} ( p - q ) -4\sigma & \mbox{(Since $b(p) \geq 1$)} \notag \\
&< e^{- \eps} ( p - q ) -3\sigma & 
  \end{align}
%\end{proof}


%\begin{claim}
%  Assume $(x,p)$ and $(y,q)$ are such that $q < p - 2\eps$. It is the case that $v\cdot \tilde{x} - v \cdot \tilde{y} \geq e^{-\eps} (v \cdot x-  v \cdot y)$.
%\end{claim}
%\begin{proof}
  \begin{align}
    v\cdot \tilde{x} - v \cdot \tilde{y} &= e^{-\eps}[ b(p) \cdot  v  \cdot  x'  - b(q) \cdot v  \cdot  y'  ] & \mbox{(By definition of  $r(.)$)} \notag\\
    &\geq e^{-\eps}[ b(p) (  e^{-\sigma} v  \cdot  x - \sigma)  - b(q) (e^\sigma v  \cdot  y + \sigma ) ] & \mbox{(By definition of  $r(.)$)} \notag\\
    &= e^{-\eps}( e^{-\sigma} b(p)    v  \cdot  x   -  e^\sigma  b(q) v  \cdot  y )  - e^{-\eps} (b(p) + b(q)) \sigma &  \notag\\
    &\geq e^{-\eps}( e^{-\sigma} b(p)    v  \cdot  x   -  e^\sigma  b(q) v  \cdot  y )  - 2 \sigma &  \mbox{(Since $b(p), b(q) \leq e^\eps $)} \notag\\
     &\geq e^{-\eps}(  e^{\sigma} b(q)  \cdot v \cdot x  - e^\sigma b(q)  \cdot v \cdot   y  ) - 2 \sigma &\mbox{(Since $b(p) \geq e^{2\sigma} b(q)$)} \notag\\
&\geq e^{-\eps}( v \cdot x  - v \cdot   y  ) - 2 \sigma & \mbox{(Since $e^\sigma b(q) \geq 1$)} \notag\\
&> e^{-\eps}( v \cdot x  - v \cdot   y  ) - 3 \sigma & 
  \end{align}
%\end{proof}
\end{proof}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pricing"
%%% End: 


==> classes.pre_cut.tex <==
\section{Upper Bounds for Structured Valuation Classes}
\label{sec:classes}
In this section, we instantiate the results in Section \ref{sec:description} by looking at two
special classes of valuations for which the computational task is tractable : \emph{monotone valuations} and \emph{monotone concave valuations}. Both classes fix an order on outcomes, without loss the order $1,\ldots,m$.  We
still assume all valuations are bounded within $[1, H]$ for some parameter $H$.

\begin{definition}
A valuations $v \in [1,H]^m$ is \emph{monotone} if $v_i \leq v_{i+1}$ for $i \in \set{1,\ldots,m-1}$. A monotone valuation is \emph{concave} if moreover $v_i - v_{i-1} \ge v_{i+1} - v_i$ for $i \in \set{1,\ldots,m-1}$, with the convention that $v_0=0$.
\end{definition}
\noindent Monotone and concave valuations  are natural in contexts such as \emph{multi-unit auctions}, where $m$ identical goods are being sold, and an outcome corresponds to the number of goods allocated to the buyer. In this setting,  $v_i$ is the player's value for $i$ goods. Monotone valuations then correspond to a free disposal assumption in multi-unit auctions, and concave valuations correspond to diminishing marginal utility.

Next we show that for concave valuations and monotone valuations, we can find
small and effective one-sided $\eps$-covers of the family of all mechanisms $\M_{\infty}$. Therefore, we can design
efficient algorithms for approximating the optimal pricing by Lemma \ref{lem:alg}. Our runtime and sample complexity guarantee is polynomial for monotone concave valuations, and quasipolynomial for monotone valuations. We summarize our findings in Theorem \ref{??}, and prove it for monotone valuations in Section \ref{}, and for monotone concave valuations in Section \ref{??}

\begin{theorem}[continues=blah]
  Monotone: $\poly(m,H)^{\frac{\log H}{\eps^2}}$
\end{theorem}

\subsection{Monotone Valuations}

\begin{definition}
Given lottery $x \in \Delta^m$, we define the tail-probability form $\bar{x} \in [0,1]^m$ of  $x$ as follows:  $\bar{x}_i = \sum_{j=i}^m x_j$.
\end{definition}

We use the fact that, for a monotone valuation $v$ and a lottery $x$, the value of the lottery can be written as follows.
\begin{align}
  \label{eq:tailval}
v.x = \sum_{i=1}^m (v_i - v_{i-1}) \bar{x}_i
\end{align}




\begin{lemma}\label{lem:lotterycover_mono}
  For every $\sigma > 0$, there is an effective (2-sided) $\sigma$-cover $\L$ of $\Delta_m$ with respect to monotone valuations, satisfying \[ |\L| \leq m^{\tilde{O}(\frac{\log H}{\sigma})}\]
\end{lemma}
\begin{proof}
The family $\L$ consists of all lotteries $y \in \Delta_m$ who's tail probability form $\bar{y}$ satisfies $\bar{y}_i \in \set{0} \union \set{ \frac{\sigma}{H} (1+ \sigma)^{t}: t \in 0,1,\ldots,\floor{\log_{1+\sigma} \frac{H}{\sigma}}}$. A simple counting argument shows that $|\L|$ satisfies the claimed bound. 
  
We show that $\L$ is an effective $\sigma$-cover by exhibiting a ``rounding algorithm'' for mapping an arbitrary $x \in \Delta_m$ to some $y \in \L$ satisfying Equation \eqref{eq:epscover_lottery}. The rounding algorithm is simple: round down each entry of the tail probability form $\bar{x}$ to the nearest number from the set $\set{0} \union \set{ \frac{\sigma}{H} (1+ \sigma)^{t}: t \in 0,1,\ldots,\floor{\log_{1+\sigma} \frac{H}{\sigma}}}$. This results in the tail probability form $\bar{y}$ of some $y \in \L$. The following calculations show that $\L$ is a $\sigma$-cover.
\begin{align}
v \cdot y &= \sum_i (v_i - v_{i-1}) \bar{y}_i  &&\mbox{(by equation \eqref{eq:tailval})} \notag \\
&\leq \sum_i (v_i - v_{i-1}) \bar{x}_i  && \mbox{(since $\bar{y}\leq \bar{x}$ entry-wise)}\notag \\
&= v \cdot x  &&\mbox{(by equation \eqref{eq:tailval})}\\ 
\notag \\
v \cdot x &= \sum_i (v_i - v_{i-1}) \bar{x}_i  &&\mbox{(by equation \eqref{eq:tailval})} \notag \\
&\leq \sum_i (v_i - v_{i-1}) \left[e^\sigma \bar{y}_i + \frac{\sigma}{H} \right]  && \notag \mbox{(by definition of $\bar{y}$)}\\
&= e^\sigma \sum_i (v_i - v_{i-1})  \bar{y}_i + \sum_i (v_i - v_{i-1}) \frac{\sigma}{H}  && \notag \mbox{}\notag\\
&= e^\sigma v \cdot y + v_m \frac{\sigma}{H}  &&\mbox{(by equation \eqref{eq:tailval})}\notag \\
&\leq e^\sigma v \cdot y + \sigma  &&\mbox{(since $v_m \leq H$)}
\end{align}
Moreover, the rounding algorithm $x \to y$ shows that $\L$ is effective.
\end{proof}

Taking $\sigma = \frac{\eps^2}{\log H}$ in Lemma \ref{lem:lotterycover_mono}, and invoking Lemma \ref{lem:lottery_to_menu_cover}, we get a one-sided $O(\epsilon)$-cover $\N$ of $\M_\infty$ with respect to monotone valuations, and $|\N| \leq \exp(m^{\tilde{O}(\log^2 H / \eps^2)})$. Instantiating Lemma \ref{lem:alg} and Algorithm \ref{alg:main} with $\N$ and $\M_\infty$ proves Theorem \ref{} for monotone valuations.



\subsection{Monotone Concave Valuations}

\begin{definition}
Given lottery $l \in \Delta^m$, define the tail-probability form of $l$ as
vector $s \in [0, 1]^m$ where $s_i = \sum_{j=i}^m x_j$.
\end{definition}
\label{submod}

Note that for a montone (or concave) valuation $v$ and a lottery $l \in
\Delta^m$, $v \cdot l$ can be rewritten as $\sum_{i=1}^m (v_i - v_{i-1})
(\sum_{j=i}^m l_j) = \sum_{i=1}^m (v_i - v_{i-1}) s_i$.


\begin{definition}[Level \& Lottery Rounding]
Given parameter $\eps$, $\delta$ and $\theta$, partition $[1..m]$ into
geometrically placed intervals $\{(a_{i - 1}, a_{i} ] \}_{i=1}^{K}$ \footnote{Assuming $a_0 = 0$ and $a_{K} = m$}
where $\frac{a_i}{a_{i-1} + 1} \le 1 + \delta$ for $i \in [K]$.
For $l \in \Delta^m$, define $l' = G_{\eps, \theta}^\delta(l)$ as follows:
\begin{enumerate}
  \item Let $y_{i} = \sum_{j = a_{i - 1} + 1}^{a_i} x_j$ for $i \in [K]$;
  \item Transform $y$ into its \text{tail-probability} form $s$,
  for each entry $s_i$ in $s$: if $s_i \ge \theta$ and $s_i \in [
  \frac{1}{(1 + \eps)^{j + 1}}, \frac{1}{(1 +
  \eps)^j}]$, then round $s_i$ up to $s_i' = \frac{1}{(1 + \eps)^j}$; 
  \item Otherwise if $s_i < \theta$, round it up to $s_i' = \theta$;
  \item Transform $s'$ back into normal form $l'$ \footnote{As $s' \in R^K$
  while $l' \in R^m$, we need pad some zeros into $l'$.};
  \end{enumerate}
  

\end{definition}

It is easy to see that $K$ is in the order of $\log_{1 +
\delta} m = \frac{1}{\delta} \log m$. Let $\mathcal{L}$ be a set of lotteries,
define $G_{\eps, \theta}^\delta(\mathcal{L}) = \{ G_{\eps, \theta}^\delta(l) :
l \in \mathcal{L} \}$.


\begin{lemma}
\label{submod_eps}
Let $\mathcal{L} = G_{\eps,\theta}^\delta(\Delta^m)$, for every lottery $l \in
\Delta^m$, there exists $l' \in \mathcal{L}$ such that $v \cdot l \le v \cdot l' \le v \cdot l (1 + \eps) (1 +
\delta) + H \theta$ for every concave
valuation $v \in [1, H]^m$.
\end{lemma}
\begin{proof}
Let $l' = G_{\eps, \theta}^\delta(l)$.
The first inequality is trivial as $G_{\eps, \theta}^\delta$ only round
probabilities up.

We analyze how $G$ works step by step to prove the second inequality. After step
$1$, $v \cdot l$ increases to $\sum_{j=1}^K v_{a_j} y_j$. By concavity, 
$\sum_{j=1}^K v_{a_j} y_j \le (1 + \delta) v \cdot l$. Note that $\sum_{j=1}^K
(v_{a_j} - v_{a_{j-1}}) s_j = \sum_{j=1}^K v_{a_j} y_j$. As $s_i$ is rounded up
to the next power of $\frac{1}{1 + \eps}$, so the increase of $\sum_{j=1}^K
(v_{a_j} - v_{a_{j-1}}) s_j$ is at most a factor of $(1 + \eps)$. After step
$3$, $\sum_{j=1}^K (v_{a_j} - v_{a_{j-1}}) s_j$ can only increase additively by
at most $H \theta$. The last step does not change the value.
\end{proof}

So $\mathcal{L} = G^{\eps^2/(2 \log H)}_{\eps^2/(2\log H), \eps^3 /
(H \log H)}(\Delta^m)$ \footnote{Note that we only need to consider cases where
$v \cdot l \ge \eps$, if $v \cdot l < \eps$ the loss in revenue in negligible.} is a $\frac{\eps^2}{\log H}$-cover
for $\Delta^m$.
Next we bound the size of $\mathcal{L}$. First, we state a result of
binomial coefficients that simplifies the analysis.

\begin{lemma}
\begin{equation}
{{a \log N + b \log N} \choose {a \log N}} \le O(N^{a \log (1 + b/a) + b \log
(1 + a/b)})
\end{equation}
\end{lemma}
\begin{proof}
By stirling approximation we have: \begin{equation}
N! = \Theta(\sqrt{N} \frac{N^N}{e^N}).
\end{equation}
So \begin{align}
{{a \log N + b \log N} \choose {a \log N}} =& \Theta(\frac{\sqrt{(a + b) \log
N} ((a + b) \log
N)^{(a + b) \log
N}}{\sqrt{a \log N} \sqrt{b \log N} (a \log N)^{a \log N} (b \log N)^{b \log
N}}) \\
\le& O((1 + \frac{b}{a})^{a \log N} (1 + \frac{a}{b})^{b \log N})
\end{align}
\end{proof}

\begin{lemma}
\begin{equation}
|\mathcal{L}| \le {{\frac{2 \log H}{\eps^2} \log m + \frac{2 \log H}{\eps^2}
\log \frac{H \log H}{\eps^3})} \choose {\frac{2 \log H}{\eps^2} \log m}} 
\end{equation}
\end{lemma}
\begin{proof}
As each lottery $l$ in $\L$ is uniquely determined by its tail-probability form
$s$ and $s_i$ has to be a power of $(1 + \frac{\eps}{2 \log H})^{-1}$ or
$\theta$.
$|\L|$ is bouned by \begin{equation}
|\{ (s_1,
s_2, \cdots, s_K) :
s_i \ge s_{i+1}, s_1 \le 1, s_K \ge \frac{\eps^3}{2H \log H}, s_i = (1 +
\frac{\eps^2}{2 \log H})^{-j} \text{ for some $j$}\} |
\end{equation}
This is equivalent to counting how many ways are there to insert $\frac{2\log
H}{\eps^2} \log \frac{H \log H}{\eps^3}$ separators into $K$ numbers, where each
separator indicates a jump in value. In particular, consider $s_K$ through $s_1$
are lined from left to right. Whenever $t$ separators is inserted between $s_i$
and $s_{i-1}$, we set $s_i = (1 + \frac{\eps^2}{2 \log H})^t s_{i-1}$.
Then the lemma follows.
\end{proof}

This means that we have found a small two-sided $\frac{\eps^2}{\log H}$-cover of
$\Delta^m$ as refered in Lemma \ref{lem:lottery_to_menu_cover1}. Moreover, the
size of this two-sided cover is polylogarthmic in $m$ where the exponent of
$\log m$ only depends on $\frac{1}{\eps}$ and $\log H$.

\subsection{Monotone Valuations}
We start by defining function $F$ which is similar to $G$ used in the concave
valuation.
\begin{definition}
Given parameter $\eps < 1$, $\theta < 1$ and $l \in \Delta^m$, 
%Without loss of generality, we assume $\theta$ is a
%power of $\frac{1}{1 + \eps^2}$. 
define $l' = F_\eps^\theta(l)$ as follows
\begin{enumerate}
  \item Transform $l$ into its tail-probabilty form $s$;
  \item If $s_i \ge \theta$ and $s_i \in [ \frac{1}{(1 + \eps)^{j+1}},
  \frac{1}{(1 + \eps)^j}]$, then round $s_i$ up to $s_i' = \frac{1}{(1
  + \eps)^j}$;
  \item If $s_i < \theta$, then round it up to $s_i' = \theta$;
  \item Transform $s'$ back into the normal form $l'$;
\end{enumerate}

Define $F_\eps^\theta(\mathcal{L}) = \{ F_\eps^\theta(l) : l \in
\mathcal{L} \}$.
\end{definition}
% Recall that $\sum_{i=1}^m v_i l_i = \sum_{i=1}^m (v_i - v_{i - 1}) (\sum_{j=i}^m
% l_j) = \sum_{i=1}^m (v_i - v_{i - 1}) s_i$\footnote{We can do this since $v$ is
% monotone.}.
\begin{lemma}
Let $\mathcal{L} = F_\eps^\theta(\Delta^m)$, then for every lottery $l \in
\Delta^m$, there exists $l' \in \mathcal{L}$ such that $v \cdot l \le v \cdot l' \le v \cdot l (1 + \eps) +
H \theta$ for every monotone valuation
$v \in [1, H]^m$ .
\end{lemma}
\begin{proof}
Similar to the proof of Lemma \ref{submod_eps}
\end{proof}

So $\mathcal{L} = F_{\eps^2/(2 \log H)}^{\eps^3/(2 \log H)}(\Delta^m)$ is a
$\frac{\eps^2}{\log H}$-cover for $\Delta^m$. Next we bound the size of
$\mathcal{L}$.
\begin{lemma}
$|\mathcal{L}| \le {{m + O(\frac{2 \log H}{\eps^2} \log \frac{2 \log H}{\eps^3})}
\choose {m}}$.
\end{lemma}
\begin{proof}
Using the same idea from the concave valuation setting. We know that the size of
$\L$ is bounded by
\begin{equation}
\mathcal{L} \le {{m + O(\frac{2 \log H}{\eps^2} \log \frac{2 \log H}{\eps^3})}
\choose {m}},
\end{equation}
which is a polynomial of $m$ for any fixed $\eps$. Moreover, the exponent of the
polynomial only depends on $ \log H$ rather than $H$.
\end{proof}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pricing"
%%% End: 


==> classes.tex <==
\section{A Special Case of Valuations}
\label{sec:classes}
%see classes.pre_cut.tex for state before submodular valuations were cut.
In this section, we instantiate the results in Section \ref{sec:description} by looking at a special class of valuations  for which the computational task is more tractable. The class we consider fixes an order on items, without loss the order $1,\ldots,m$. A valuation $v \in [1,H]^m$ is \emph{monotone} if $v_i \leq v_{i+1}$ for $i \in \set{1,\ldots,m-1}$.  Monotone valuations  are natural in contexts such as \emph{multi-unit auctions}, where $m$ identical goods are being sold, and an outcome corresponds to the number of goods allocated to the buyer. In this setting,  $v_i$ is the player's value for $i$ goods. Monotone valuations then correspond to a free disposal assumption in multi-unit auctions.

Next we show that for  monotone valuations, we can find a
small and effective one-sided $\eps$-cover $\N$ of the family of all mechanisms $\M_{\infty}$ with respect to monotone valuations. Moreover, every menu in $\N$ has a small number of entries. Therefore, we can design an
efficient algorithm for approximating the optimal pricing by Lemma \ref{lem:alg}. Our runtime, menu complexity, and sample complexity guarantee is polynomial in $m$ when $H$ is a constant, and quasipolynomial when $H$ grows polynomially with $m$. We prove the following theorem.

\begin{theorem}\thmcontinues{thm:monotone}
If $\D$ is supported on monotone valuations then for every $\epsilon>0$ there exists a menu $M$ with $m^{\tilde{O}(\frac{\log^2 H}{\eps^2})}$ entries such that 
$Rev(M,\D) \ge (1-\epsilon) Rev(\D)$.   Furthermore,  such a menu can be computed in time $m^{\tilde{O}(\frac{\log^2 H}{\eps^2})}$.
\end{theorem}
\noindent Our proof of Theorem \ref{thm:monotone} relies on the following Lemma






\begin{lemma}\label{lem:lotterycover_mono}
  For every $\sigma > 0$, there is an effective (2-sided) $\sigma$-cover $\L$ of $\Delta_m$ with respect to monotone valuations, satisfying \[ |\L| \leq m^{O(\frac{\log H}{\sigma} + \frac{1}{\sigma} \log \frac{1}{\sigma})}\]
\end{lemma}
\begin{proof}
Given lottery $x \in \Delta^m$, we define the tail-probability form $\bar{x} \in [0,1]^m$ of  $x$ as follows:  $\bar{x}_i = \sum_{j=i}^m x_j$. We use the fact that, for a monotone valuation $v$ and a lottery $x$, the value of the lottery can be written as follows.
\begin{align}
  \label{eq:tailval}
v.x = \sum_{i=1}^m (v_i - v_{i-1}) \bar{x}_i
\end{align}


The family $\L$ consists of all lotteries $y \in \Delta_m$ who's tail probability form $\bar{y}$ satisfies $\bar{y}_i \in \set{0} \union \set{ \frac{\sigma}{H} (1+ \sigma)^{t}: t \in 0,1,\ldots,\floor{\log_{1+\sigma} \frac{H}{\sigma}}}$. A simple counting argument shows that $|\L|$ satisfies the claimed bound. 
  
We show that $\L$ is an effective $\sigma$-cover by exhibiting a ``rounding algorithm'' for mapping an arbitrary $x \in \Delta_m$ to some $y \in \L$ satisfying Equation \eqref{eq:epscover_lottery}. The rounding algorithm is simple: round down each entry of the tail probability form $\bar{x}$ to the nearest number from the set $\set{0} \union \set{ \frac{\sigma}{H} (1+ \sigma)^{t}: t \in 0,1,\ldots,\floor{\log_{1+\sigma} \frac{H}{\sigma}}}$. This results in the tail probability form $\bar{y}$ of some $y \in \L$. The following calculations show that $\L$ is a $\sigma$-cover.
\begin{align}
v \cdot y &= \sum_i (v_i - v_{i-1}) \bar{y}_i  &&\mbox{(by equation \eqref{eq:tailval})} \notag \\
&\leq \sum_i (v_i - v_{i-1}) \bar{x}_i  && \mbox{(since $\bar{y}\leq \bar{x}$ entry-wise)}\notag \\
&= v \cdot x  &&\mbox{(by equation \eqref{eq:tailval})}\\ 
\notag \\
v \cdot x &= \sum_i (v_i - v_{i-1}) \bar{x}_i  &&\mbox{(by equation \eqref{eq:tailval})} \notag \\
&\leq \sum_i (v_i - v_{i-1}) \left[e^\sigma \bar{y}_i + \frac{\sigma}{H} \right]  && \notag \mbox{(by definition of $\bar{y}$)}\\
&= e^\sigma \sum_i (v_i - v_{i-1})  \bar{y}_i + \sum_i (v_i - v_{i-1}) \frac{\sigma}{H}  && \notag \mbox{}\notag\\
&= e^\sigma v \cdot y + v_m \frac{\sigma}{H}  &&\mbox{(by equation \eqref{eq:tailval})}\notag \\
&\leq e^\sigma v \cdot y + \sigma  &&\mbox{(since $v_m \leq H$)}
\end{align}
Moreover, the rounding algorithm $x \to y$ shows that $\L$ is effective.
\end{proof}

Taking $\sigma = \frac{\eps^2}{\log H}$ in Lemma \ref{lem:lotterycover_mono}, and invoking Lemma \ref{lem:lottery_to_menu_cover}, we get a one-sided $O(\epsilon)$-cover $\N$ of $\M_\infty$ with respect to monotone valuations, and $|\N| \leq \exp(m^{\tilde{O}(\log^2 H / \eps^2)})$. Instantiating Lemma \ref{lem:alg} and Algorithm \ref{alg:main} with $\N$ and $\M_\infty$ proves Theorem \ref{thm:monotone}.




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pricing"
%%% End: 


==> complexity.tex <==
\section{Lower Bounds on Menu Complexity}
\label{sec:complexity}
In this section, we show that there exist distributions $\D$ over unit-demand valuations for which any near-optimal pricing mechanism is necessarily ``complex''.  We quantify the complexity of a menu by its size, though we believe that our results are robust to the choice of complexity measure.

\begin{note}
There are a couple of questions we need to answer:
\begin{itemize}
\item We need to argue convincingly that the size of a menu is a ``useful'' complexity measure in this context. Does a large menu size rule out mechanisms that sample $\D$ and produce an outcome and allocation ``on the fly''? Noam mentioned to me that his lower bound rules out good mechanisms with any short description, though I don't recall the details. We need to think carefully about what the result below implies for the intractability of the pricing problem in the black box oracle model.
\item Li established lower bounds on the Radermacher Complexity of pricing mechanisms. These lowerbounds are closely related to the ``sample complexity'' of fitting a mechanism to samples from $\D$. I'm not quite sure yet how to connect these lowerbounds to the menu-size results, so I'm relegating them to Appendix \ref{sec:radermacher} for now (I did not edit that section yet, so there might be some notational inconsistencies in the appendix). We need to think about whether these results are interesting and add something to the story, and if so what.
\end{itemize}


\end{note}

\begin{theorem}\label{thm:menu_complexity}
Fix an arbitrary integer $ H$.  There exists a distribution $\D$ supported on $[1,H]^m$ such that, for all $k$, \[ \frac{\Rev(\D)}{\Rev_k(D)} \geq \Omega (\min(\log H, \frac{\exp(m)}{k}))\]
\end{theorem}

\begin{proof}
  TODO
\end{proof}

\begin{note}
  I'm not sure if I got the above bound exactly right. I'll leave the proof till after we discuss with Noam. Also, to motivate some of the stuff of Section \ref{sec:small}, I think it would be a good idea to prove a lower bound parametrized by two different menu sizes --- i.e. For every $k,k'$ with $k \leq k' \leq  \exp(m)$, there is a distribution $\D$ supported on $[1,H]^m$ such that $\frac{\Rev_{k}(\D)}{\Rev_{k'}(\D)} \leq \min(\log H, \frac{k}{k'})$.
\end{note}



In light of this impossibility result, we examine the optimal unit-demand pricing problem under two different forms of simplifying assumptions.  In Section \ref{sec:small}, we examine the complexity of designing an approximately optimal \emph{small} menu for an arbitrary distribution $\D$. In Section \ref{sec:classes}, we restrict the class $\V$ from which the buyer's valuation is drawn, but otherwise make no assumptions on the distribution $\D$.





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pricing"
%%% End: 


==> description.tex <==
\section{Description and Sample Complexity}
\label{sec:description}

In this section, we examine the description and sample complexity of approximate revenue maximization for distributions supported on $[1,H]^m$. Our results hold for both models of description complexity: Kolmogorov complexity and menu complexity. 
We begin by showing that, information theoretically, a bound on description complexity of the saught mechanism leads to a polynomially-related bound on the sample complexity.
First, we need the following Lemma.


\begin{lemma}\label{lem:lotterycover_all}
  For every $\sigma > 0$, there is an effective (2-sided) $\sigma$-cover $\L$ of $\Delta_m$ with respect to valuations $[1,H]^m$ with $|\L| \leq (O(\frac{1}{\sigma}\cdot (\log m + \log H +  \log \frac{1}{\sigma}))^m$.
\end{lemma}
\begin{proof}
  We let $\L$ be the family of all lotteries $x \in \Delta_m$ such that every non-zero entry $x_i$ equals $\frac{\sigma}{m H} e^{\sigma t} $ for some integer $t$. A simple counting argument shows that $|\L|$ satisfies the claimed bound. To see that $\L$ is a $\sigma$-cover, consider rounding down each entry of a lottery $x \in \Delta_m$ to the nearest number in $\set{\frac{\sigma}{m H} e^{\sigma t} : t \in \NN} \union \set{0}$ . Let $\hat{x}$ denote the image of this rounding when applied to $x$, and note that $\hat{x} \in \L$. It is easy to verify that $\hat{x}_i \leq x_i \leq e^\sigma \hat{x}_i + \frac{\sigma}{m H}$. To conclude that $\L$ is a $\sigma$-cover, observe that the following holds for every $v \in [1,H]^m$.

  \begin{align*}
v \cdot \hat{x} &\leq v \cdot x \\
&\leq e^\sigma v \cdot \hat{x} + \sum_{i=1}^m v_i \frac{\sigma}{m H} \\ 
&\leq e^\sigma v \cdot \hat{x}  + \sigma 
  \end{align*}
%
Finally, the mapping $x \to \hat{x}$ proves that $\L$ is effective.
\end{proof}



\begin{theorem}\thmcontinues{thm:smallmech}
For every $\epsilon> 0$ and distribution $\D$ supported on $[1,H]^m$, there is an algorithm which takes  $n=\poly(m,H,C,\frac{1}{\epsilon})$  samples from $\D$ and outputs a mechanism $M$ of complexity at most $C$ and revenue at least $(1-\eps)\Rev_C(\D)$, with high probability. This holds in both the Kolmogorov complexity and menu complexity models.
\end{theorem}
\begin{proof}
In the Kolmogorov complexity model, the proof of this fact is elementary. Specifically, the following ``obvious'' algorithm works: take $n$ i.i.d samples $X$ from $\D$, and return the mechanism of Kolmogorov complexity at most $C$ which maximizes revenue on the empirical distribution $X$. Correctness of this algorithm follows from uniform-convergence of the empirical estimate of revenue, over all mechanisms of complexity at most $C$. Formally, we show that the revenue of $M$ on $X$ approximates its revenue on $\D$, to within an additive $\epsilon \Rev_C(\D)$,  simultaneously for all $2^C$ mechanisms $M$ of Kolmogorov complexity bounded by $C$, with high probability.  Since valuations lie in $[1,H]$, we are guaranteed that $\Rev_C(\D) \geq 1$, so it suffices to bound the additive error by $\epsilon$ instead. For every $\delta > 0$, the Hoeffding bound and the union bound imply that $\poly(H,C,\frac{1}{\eps},\log(\frac{1}{\delta}))$ samples suffice for this guarantee to hold with probability $1-\delta$.

In the menu complexity model, the same approach does not appear to work. For one,  there is an infinite set of menus with $\leq C$ entries, so we can not apply convergence bounds such as the Hoeffding bound. This is also related to the absence of a finite $2$-sided cover of the family of $C$-menus, as described in Appendix \ref{app:nocover}. Nevertheless, the machinery of one-sided $\epsilon$-covers presented in Section \ref{sec:covers} allows us to restrict attention to a finite set $\N$ of $C$-menus which is guaranteed to contain a near optimal $C$-menu, and over which uniform convergence is guaranteed. Taking $\sigma = \frac{\eps^2}{\log H}$ in Lemma \ref{lem:lotterycover_all}, and invoking Lemma \ref{lem:lottery_to_menu_cover}, we get a one-sided $O(\epsilon)$-cover $\N_C$ of $\M_C$ with cardinality $|\N| \leq (\poly(\log H, \frac{1}{\eps}, \log m))^{m C}$. Instantiating Lemma \ref{lem:alg} and Algorithm \ref{alg:main} with $\N_C$ and $\M_C$ completes the proof.
\end{proof}




We note that a weak ``converse'' of Theorem \ref{thm:smallmech} is immediate: a lower bound of $C$ on the Kolmogorov complexity of an approximately optimal mechanism leads to a lowerbound of $C$ on the number of bits in the sample of any algorithm identifying  such a mechanism. Theorem \ref{thm:smallmech} motivates us to prove upper bounds on the  description complexity of (approximately) revenue maximizing auctions, as such upper bounds extend to the sample complexity of identifying a near optimal mechanism. For an arbitrary good approximation, our bound is exponential in the number of items, yet polynomial in $\log H$ and the desired precision.

\begin{theorem}\thmcontinues{thm:menusize}
For every $\epsilon> 0$ and distribution $\D$ supported on $[1,H]^m$,  there exists a menu $M$ with at most $\left(\tilde{O}\left(\frac{\log H}{\epsilon}\right)\right)^{\tilde{O}(m)}$ entries 
so that $\Rev(M,\D) \ge (1-\epsilon) \Rev(\D)$.%  Moreover, all real numbers in $M$ are rational numbers of at most $poly(H, \epsilon^{-1}, m)$ bits each.
\end{theorem}
\begin{proof}
This follows directly from Lemmas \ref{lem:lotterycover_all} and \ref{lem:lottery_to_menu_cover}.
\end{proof}
\noindent On the other hand, $m$ entries suffice for an $O(\log H)$ approximation. 

\begin{proposition}
For every distribution $\D$ there exists an auction with $m$ menu-entries
(and with all numbers represented in $O(\log H)$ bits)
that extracts $\Omega(1/\log H)$ fraction of the optimal revenue 
from $\D$.  
Furthermore, this auction can be computed in polynomial time from $\poly(H)$ samples.
\end{proposition}


\begin{proof}
Let $M^p$ denote the $m$-entry menu which offers every item for a price of $p$; i.e. $M^p = \{(e_i, p) : i \in \set{1,\ldots,m}\}$, where $e_i$ is the $i$'th standard basis vector. One of the $\log H$ menus $M^1, M^2, M^4, \ldots, M^H$ is guaranteed to extract a $1/2\log H$ fraction expected maximum value for an item $\Ex_{v \sim D} \max_i v_i$, which in turn is an upper bound on the maximum revenue. 

To make this algorithmic, observe that the revenue of each of $M^1, M^2, M^4, \ldots, M^H$ is a random variable between $0$ and $H$.  The algorithm is the obvious one: take $n=\omega(H^2 \log \log H)$ samples from $\D$, and return the menu from $M^1, M^2, M^4, \ldots, M^H$  with the greatest expected revenue on the sample. By applying the Hoeffding bound and the union bound, our estimate for the revenue of each menu $M^p$ is within an additive error of $1/2$ with high probability. Since $\Rev(\D) \geq 1$, the chosen menu satisfies the claimed bound.
\end{proof}


We note  that Theorem \ref{thm:menusize} and Proposition \ref{prop:logH}, though posed in the menu complexity model, hold for the Kolmogorov complexity model as well to within a $\poly(\log H, \frac{1}{\eps},m)$ factor --- we omit the details, which require modifications to Section \ref{sec:covers} involving tedious accounting of numerical precision. Finally, we show that the bounds in  Theorem \ref{thm:menusize} and Proposition \ref{prop:logH} can not be significantly improved. We prove this impossibility result in the Kolmogorov complexity model, though it extends to the menu complexity model as well.

\begin{theorem}\thmcontinues{thm:kolmogorov}
For every $1 < H < 2^{m/400}$ There exists a distribution $\D$ on $[1..H]^m$ such that for every mechanism $M$ with Kolmogorov complexity at most 
$2^{m/400}$ we have that $\Rev(M,\D) = O(1/\log H) \cdot \Rev(\D)$.
\end{theorem} 

\begin{proof}
We will construct the distribution $\D$ probabilistically.  

Our starting point will be a fixed baseline distribution $\B$ that takes an ``equal
revenue'' one-dimensional distribution and spreads it symmetrically over a random subset of the items.  
Each valuation in the support of $\B$ is specified by a set $S \subset \{1..m\}$ of size exactly $k=m/3$ and an integer scale value 
$1 \le z \le \log H$.  The valuation will give value $2^z$ for every item in $S$ and value 1 for every other item.
The probability distribution over these is induced by choosing $S$ uniformly at random among sets of size $k$ and choosing $z$ as to obtain an
``equal revenue distribution'' $Pr[z=x]=2^{-x}$.  We can view this distribution over the $v$'s as choosing a item uniformly at random from a multi-set $V$
of exactly ${\binom{m}{k}} (H-1)$ valuations (for every set $S$ of size $k$ we have $H/2$ copies of a valuation with value $2$, $H/4$ copies of a valuation
with value $4$ ... and a single copy of a valuation with value $H$). The point is that due to symmetry, it can be shown that,
just like in the corresponding the single dimensional case, $\Rev(\B)$ is constant (despite the expected value being $O(\log H)$).  This is proven formally
in lemma \ref{revB} below.

Taking the point of view of $\B$ being a random choice of a valuation from the multi-set $V$, we will now construct our distribution $\D$
as being a uniform choice over a random subset $V'$ of $V$, where $V'$ is of size $|V'|=K=2^{m/100}$.  We will now 
be able to provide two estimates.  On one hand, since $V'$ is a random sample from $V$, we expect that every fixed mechanism will extract approximately
the same revenue from $\D$ as from $\B$.  This can be shown to hold, w.h.p., simultaneously for {\em all} mechanisms in a 
small enough family and thus all 
mechanisms with sub-exponential Kolmogorov Complexity can only extract constant revenue.  On the other hand, as $V'$ is sparse, w.h.p. it does not contain
two valuations whose subsets have a large intersection.  This will suffice for extracting at east half of the expected value as revenue, an expected value that
is $O(\log H)$.  Lemma \ref{revDlow} below proves the former fact and lemma \ref{revDhigh} below proves the latter.
\end{proof}


\begin{lemma}\label{revB}
Let $\B$ denote the distribution above then $\Rev(\B) \le 2$.
\end{lemma}

\begin{proof}
We will prove this by reduction the the single dimensional case where Myerson's theorem can be used.
Let us define the single dimensional distribution $\G$ that gives value $2^x$ with probability $2^{-x}$
for $x \in \{1 ... \log H\}$.  The claim is that $Rev(\B) \le \Rev(\G) \le 2$.  Since $\G$ is single dimensional, the
second inequality follows from Myerson's result stating that a single price mechanism
maximizes revenue, as it is easy to verify that every possible single price gives revenue of at most 2.

To prove the first claim we will build a single-parameter mechanism for $\G$ with the same revenue as a given multidimensional one for $\B$.
Given a value $2^x$ distributed as in $\G$, our mechanism chooses a random
subset $S$ of size $k$ and constructs a valuation $v$ by combining the given single-parameter value with this set, so now $v$ is distributed according to $\B$. 
We run the mechanism that was given to us for $\B$ and when it returns  
an lottery $a=a(v)$, we sell the item in the single parameter auction with probability $\sum_{j \in S} a_j$, asking for the same payment as asked for 
the lottery $a$ in the $\B$-auction.  Now notice that the same outcome that maximizes utility for $v$ also maximizes utility for the single parameter buyer.
\end{proof}


\begin{lemma}\label{revDlow}
Let $\M$ be the set of mechanisms with Kolmogorov complexity at most $2^{m/400}$ and choose the distribution $\D$ 
as described above then, w.h.p., $\Rev(\M,\D) \le 3]$.
\end{lemma}

\begin{proof}
Since there are at most $2^{2^{m/400}}$ mechanisms in $\M$, this follows from the following lemma and the union bound.
\end{proof}


\begin{lemma}
Fix some mechanism $M$ and choose the distribution $\D$ 
as described above then $Pr[\Rev(M,\D) > 3] \le exp(-K/H^2) \le 2^{-2^{m/300}}$.
\end{lemma}

\begin{proof}
Let $r_M(v)$ denote the revenue that mechanism $M$ extracts on valuation $v$.
By definition $Rev(M,\B) = E_{v \in V} r_M(v)$ while $Rev(M,\D) = E_{v \in V'} r_M(v)$ (where the distribution is uniform
over the multi-sets $V$ and $V'$ respectively).  Lemma \ref{revB} bounded the former: $Rev(M,\B) \le 2$.  
Since we are choosing $V'$ to be a 
random multi-set of size $K$ and since for all $v$ we have $0 \le r_M(v) \le H$ then we can use Chernoff bounds
to bound the probability that the expectation of $r_M(v)$ over the
sample $V'$ is larger than its expectation over the population $V$ to be
$Pr [|E_{v \in V'} r_M(v) - E_{v \in V} r_M(v)| > 1] \le exp(-K/H^2)$.
\end{proof}



\begin{lemma} \label{revDhigh}
Choose the distribution $\D$ as described above then, w.h.p, $\Rev(\D) \ge \log H / 2$.
\end{lemma}

\begin{proof}
We will use the following property that holds, w.h.p., for $V'$: for every two different valuations in $V'$ the sets of items $S$ and $T$ 
associated with them satisfy $|S \cap T| < m/6$.  The reason that this property holds is
that for any fixed $T$, since $S$ is a random set of size $m/3$ the probability that
$|S \cap T| / |T| \ge 1/2$ is $exp(-|T|) \le 2^{-m/40}$.  Now we can take a union bound over all $K^2 = 2^{m/50}$
possible pairs of $S$ and $T$. 

Using this property of $\D$ here is a mechanism that extracts as revenue at least half of the expected value of $v$, i.e. at least $(\log H)/2$ revenue:
we have a menu entry for each element $v \in V'$.  For
$v$ that gives value $2^z$ to the set $S$, this entry will
offer every item in $S$ with probability $1/|S| = 3/m$, and will ask for payment of $2^{z-1}$ for this lottery.
Clearly if $v$ chooses this entry it gets net utility of exactly $2^{z-1}$, we need to show that the net utility from any
other menu entry is less than this.  Observe that $v$'s value from a menu entry that corresponds
to a set $T$ is exactly $2^z \cdot |S \cap T| / |T|$ which due to our property is bounded from above by $2^{z-1}$.
\end{proof}








%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pricing"
%%% End: 


==> nets.additive.tex <==
\section{Covers and Sample Complexity}
\label{sec:covers}


\begin{note}(Shaddin)
  \begin{itemize}
  \item Currently, results are stated in additive form, with $[0,H]$ valuations. Need to switch to multiplicative and $[1,H]$, since it seems we really need that...
  \end{itemize}
\end{note}


Our primary tool for bounding the sample complexity of pricing problems, and consequently their computational complexity, is reminiscent of $\epsilon$-covers of a metric space, though importantly different. Specifically, our positive results involve identifying a small (say, exponential) family of menus which is guaranteed to include a near optimal menu from the larger family of interest. For our applications, we use the following (strong) definition.


\begin{definition}
  Let $\N$ and $\M$ be two families of menus with $\N \sse \M$, and $\V \sse [0,H]^m$
  \footnote{For ease of presentation, we write $H$ as a constant here. Our
  techniques permit $H$ to depend polynomially on $m$.} a family of valuations.
  We say $\N$ is a \emph{one-sided $\epsilon$-cover} of $\M$ with respect to $\V$ if for every $M \in \M$ there is $N \in \N$ such that for all $v \in \V$ \begin{align}\label{eq:epscover}\Rev(N,v) \geq \Rev(M,v) - \epsilon.\end{align} We say the cover is \emph{effective} if there is an algorithm  which takes as input any finite $M \in \M$ and outputs $N \in \N$ with $|N| \leq |M|$ satisfying \eqref{eq:epscover} in time $\poly(|M|,m,\frac{1}{\eps})$.
\end{definition}



We now take a moment to reflect on this definition, and its relation to the traditional notion of an $\epsilon$-cover of a metric space. In the ensuing discussion, think of $\M$ as $\M_\infty$, the family of all menus, as is the case for our applications in Section \ref{}. One can think of every menu (i.e. mechanism)  $M$ as a function  mapping valuations $v \in \V$ to the revenue generated by the auctioneer. Viewed thus, the $\ell_\infty$ metric on the resulting function space serves as a natural distance function on menus. A (2-sided) $\epsilon$-cover of the metric space of menus, if a small one exists, guarantees that a small number of samples suffice to estimate the expected revenue of \emph{every} menu simultaneously to within a small additive error. Such a guarantee, often referred to as \emph{uniform convergence},  bounds the sample complexity of finding an approximately optimal mechanism for a hidden distribution $\D$ on $\V$ presented as an oracle. When uniform convergence holds, the optimal mechanism on the sample is approximately optimal on the hidden distribution, with high probability. In effect, uniform convergence reduces finding the optimal mechanism for the hidden distribution to finding the optimal mechanism for the sample, in analogy to \emph{empirical risk minimization} in PAC learning. Uniform convergence guarantees are commonplace in the machine learning literature, and have even been suggested and applied to optimal mechanism design by Balcan et al \cite{}. However, as we show in Section \ref{}, finite $\epsilon$-covers in the classical (i.e., 2-sided) sense do not exist for the space of pricing mechanisms, even in the special case of pricing a single item. This observation motivates our weaker definition.


If a family  $\M$ of menus admits a small one-sided $\epsilon$-cover $\N$ with respect to $\V$, and $\D$ is supported on $\V$, we can still bound the number of samples necessary for identifying a near optimal menu in $\M$. Specifically, using well-known concentration inequalities and the union bound, we conclude that $\log |\N|$ samples from $\D$ suffice for approximately estimating  $\Rev(N,\D)$ for every $N \in \N$. Whereas we can not make such a guarantee for every menu $M \in \M$ in the larger class, we do not need to, since  some $N \in \N$ is approximately optimal! There is one quirk of this approach, due to the fact that our $\epsilon$-cover is one sided: it no longer suffices to output the revenue-maximizing menu using the sampled valuations, as such a menu may not lie in $\N$, and may therefore have revenue that differs substantially from that estimated by our sample. Our algorithm must in fact output a menu in the cover $\N$ to avoid \emph{over-fitting} to the sample.\footnote{Our technique of fitting an element of a small cover of all menus can be thought of as a discrete variant of \emph{regularization}, a technique thoroughly employed in the machine learning community.} This is OK for an information theoretic result, but introduces a computational challenge for our applications: when $\M=\M_\infty$ is the space of all menus, finding an optimal unconstrained menu for an explicitly given distribution (the sample) reduces to solving a simple linear program. The same cannot be said of the finite covers $\N$ we construct. Fortunately, we show below that it suffices to exhibit an efficient ``rounding procedure'' which maps menus in $\M$ to menus in $\N$, as doing so recovers computational tractability. We summarize these observations in Algorithm \ref{alg:main} and Lemma \ref{lem:alg}.


\begin{algorithm}
\caption{Sample \& Round Pricing Algorithm}
\label{alg:main}
\begin{algorithmic}[1]
  \PARAMETER Family $\V \sse [0,H]^m$ of valuations
  \PARAMETER Family $\M$ of menus
  \PARAMETER An $\epsilon$-cover $\N$ of $\M$ with respect to $\V$
  \INPUT Distribution $\D$ with support $\V$, presented as a black box
  \OUTPUT $N \in \N$ satisfying $\Rev(N,\D) \geq \Rev(M,\D) - \epsilon$ for every $M \in \M$, with high probability
  \STATE Sample $n = \poly(m, H, \log |\N|, \frac{1}{\eps})$ times from $\D$,
  denote the samples by $S = \{ v_1, \cdots, v_n \}$;
  \STATE Let $M_S\in \argmax_{M \in \M} \Rev(M,S)$ 
  \STATE Let $N_S \in \N$ satisfy $\Rev(N_S,v) \geq \Rev(M_S,v) - \eps$ for every $v \in \V$ (Equation \eqref{eq:epscover})
  \STATE Output $N_S$
  \end{algorithmic}
\end{algorithm}


\begin{lemma}\label{lem:alg}
  If $\N$ is a one-sided $\epsilon$-cover of $\M$ with respect to $\V \sse
  [0, H]^m$, then Algorithm \ref{alg:main} outputs $N \in \N$ such that $\Rev(N,\D) \geq \Rev(\M,\D) - 3\eps$ for every $M \in \M$, with high probability. Moreover, when $\M=\M_\infty$ and $\N$ is an effective cover, Algorithm \ref{alg:main} runs in $\poly(m, H, \log |\N|, \frac{1}{\eps})$ time.
\end{lemma}
\begin{proof}
We begin by showing that the sample $S$ provides an estimate, within an additive $\epsilon$, of the revenue of every menu $N \in \N$.  For any fixed $N \in \N$, by the Hoeffding bound we have $Pr[|\Rev(N, \D) - \Rev(N,S)| > \eps] \le 2e^{-\frac{2n \eps^2}{H^2}}$. Applying the union bound, we get 
  \begin{equation}
  Pr[\exists N \in \N \text{ s.t. } \Rev(N, \D) - \Rev(N,S)| > \eps] \le 2
  e^{-\frac{2n \eps^2}{H^2}} |\N|
  \end{equation}
  So when the number of samples $n$ is  $poly(m, H, \frac{1}{\eps}, \log |\N|)$, the empirical revenue of every menu in $\N$ approximates its revenue on $\D$, with high probability.
  

Let $M^*$ be an optimal menu for distribution $\D$. Using the Hoeffding bound again, we conclude that $|\Rev(M^*, S) - \Rev(M^*, \D )| \leq \epsilon$ with high probability --- i.e. the empirical revenue of $M^*$ approximates its revenue on $\D$. The following holds with high probability, completing the proof of the approximation guarantee.
\begin{align*}
  \Rev(N_S, \D) &\geq \Rev(N_s,S) - \eps \\
  &\geq \Rev(M_s, S) - 2\eps \\
  &\geq \Rev(M^*,S) -2\eps \\
  &\geq \Rev(M^*,\D) - 3\eps
\end{align*}


We now analyze the runtime of this algorithm when $\M=\M_\infty$ and $\N$ is effective.  Recall that step 2 reduces to solving a linear program with $O(nm)$ variables, and outputs a menu $M_S$ with $|M_S| \leq n$. Step 3 then runs in $\poly(n,m)$ time, since $\N$ is effective. 
  
\end{proof}
Algorithm \ref{alg:main}  and Lemma \ref{lem:alg} reduce the design of algorithms for pricing problems to the design of small one-sided $\epsilon$-covers of menu families. 
Our main technique for constructing one-sided $\epsilon$-covers of
menus is through constructing a two-sided $\eps$-covers of the set of lotteries, defined below.

\begin{definition}
  A family $\L \sse \Delta_m$ of lotteries is a (two-sided) $\epsilon$-cover of $\Delta_m$ with respect to $\V$ if for every $x \in \Delta_m$ there is $y \in \L$ such that the following holds for all $v \in \V$ \begin{align}\label{eq:epscover_val} |v \cdot x - v\cdot y| \leq  \eps\end{align} Moreover, we say the cover is \emph{effective} if there is an algorithm which takes as input $x \in \Delta_m$ and outputs $y \in \L$ satisfying \eqref{eq:epscover_val} in time $\poly(m,\frac{1}{\eps})$
\end{definition}




\begin{lemma}\label{lem:lottery_to_menu_cover1}
  If $\L$ is an $\epsilon^2$-cover of $\Delta_m$ with respect to $\V \sse
  [0,H]^m$, then there is a one-sided $6\eps$-cover
  $\N$ of $\M_k$ with respect to $\V$ with $|\N| \leq \min\left\{\left(\frac{H}{\eps^2}\right)^{|\L|}, \left(\frac{H|\L|}{\eps^2}\right)^k \right\}$.
  Moreover, if $\L$ is effective, then so is $\N$.
\end{lemma}
\noindent We note that when $k=\infty$, the guarantee on the size of $\N$ simplifies to $\left(\frac{H}{\eps^2}\right)^{|\L|}$

\begin{proof}

For each $M \in \M$, include in $\N$ an approximation $\tilde{M}$ of $M$, defined as follows. For every $(x,p)$ in $M$, include in $\tilde{M}$ an entry  $(\tilde{x},\tilde{p})$ satisfying:
\begin{itemize}
\item $\tilde{x} \in \L$ and $|v \cdot x - v \cdot \tilde{x} | \leq \eps^2$ for every $v \in \V$ 
\item Let $t \eps^2$ be the result of rounding down $p$ to the nearest integer multiple of $\eps^2$, and let $\tilde{p}= t (\eps^2 - \eps^3) $
\end{itemize}
Since at most $\frac{H}{\eps^2}$ different prices and  $|\L|$ different lotteries appear in $\N$, we have that $|\N| \leq \left(\frac{H}{\eps^2}\right)^{|\L|}$.  Moreover, since every $N \in \N$ has at most $k$ entries, each of which is a lottery in $\L$ and a price, we have that $|\N| \leq \left(\frac{H|\L|}{\eps^2}\right)^k$.


We now claim that $\Rev(M, v) - \Rev(\tilde{M},v) \leq 6 \eps$ for every $v \in \V$. Intuitively,  the mapping $(x,p) \to (\tilde{x},\tilde{p})$ described above changes a player's value for allocation $x$ by at most $\eps^2$, and reduces the price $p$ by a quantity between $\eps^2$ and $ \eps+\eps^2$ which increases as $p$ increases. This increasing discount for pricy lotteries makes them comparatively more attractive, limiting the decrease in revenue. Formally, for $(x,p) \in M$, we can bound the change of utility  $(v \cdot \tilde{x} - \tilde{p}) - (v \cdot x - p)$ as follows.
\begin{align*}
  p\eps + 2 \eps^2 \geq  \floor{p/\eps^2} \eps^3 + 2\eps^2  \geq (p-\tilde{p}) - (v \cdot x - v\cdot \tilde{x})  
\geq \floor{p/\eps^2} \eps^3 - \eps^2 \geq p \eps - 2 \eps^2
\end{align*}

Now assume that a buyer $v$ buys lottery $(x,p) \in M$, and $(\tilde{y},\tilde{q}) \in M'$. 
%
%
\begin{align*}
v \cdot y - q  &\leq v \cdot x - p \\ 
v \cdot \tilde{y} - \tilde{q}  &\geq v \cdot \tilde{x} - \tilde{p} \\
q\eps + 2 \eps^2 \geq (v \cdot \tilde{y} - \tilde{q}) - (v \cdot y - q)&\geq (v \cdot \tilde{x} - \tilde{p}) - ( v \cdot x - p) \geq p\eps - 2 \eps^2  \\
q\geq p - 4 \eps \\
\end{align*}

Since $\tilde{q} \geq q - \eps - \eps^2$, we conclude that $\tilde{q} \geq p - 6 \eps$, establishing that $\N$ is a one-sided $\epsilon$-cover of $\M$. Moreover, when $\L$ is effective, the mapping $M \to \tilde{M}$ is proof that $\N$ is effective.
\end{proof}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pricing"
%%% End: 


==> nets.multiplicative.tex <==
\section{Nets and Sample Complexity}
\label{sec:nets}


% \begin{note}
% %  At some point should move to $[1,H]$ valuations. Also, 
% should fill in the story.
% \end{note}


\begin{definition}
  Let $\N$ and $\M$ be two families of menus, and $\V \sse \RRp^m$ a family of valuations. We say $\N$ is a \emph{one-sided $\epsilon$-net} of $\M$ with respect to $\V$ if for every $M \in \M$ there is $N \in \N$ such that for all $v \in \V$ \begin{align}\label{eq:epsnet}\Rev(N,v) \geq (1-\eps) \Rev(M,v) .\end{align} We say the net is \emph{effective} if there is an algorithm  which takes as input $M \in \M$ and outputs $N \in \N$ with $|N| \leq |M|$ satisfying \eqref{eq:epsnet} in time $\poly(|M|,m)$.  
\end{definition}



\begin{theorem}\label{thm:nets1}
  If $\N$ is a finite one-sided $\epsilon$-net of $\M_\infty$ with respect to $\V \sse [1,H]^m$, then there is high probability $(1-\eps)$-approximation algorithm for the pricing problem in the black box model which makes $n=\poly(m,\log |\N|, H)$ queries. Moreover, if the net is effective, then the algorithm runs in time polynomial in $n$.
\end{theorem}
\begin{proof}

\end{proof}

\begin{theorem}\label{thm:nets2}
  If $\N$ is a finite one-sided $\epsilon$-net of $\M$ with respect to $\V \sse [1,H]^m$, then there is an algorithm for the pricing problem in the black box model which makes $n=\poly(m,\log |\N|, H)$ queries, and outputs $N \in \N$ such that $\Rev(N,\D) \geq (1-\eps) \Rev(\M,\D)$.
\end{theorem}
\begin{proof}
  
\end{proof}


Our main technique for constructing $\epsilon$-nets of menus is through constructing an $\eps$-net of the set of lotteries.

\begin{definition}
  A family $\L \sse \Delta_m$ of lotteries is a (two-sided) $\epsilon$-net of $\Delta_m$ with respect to $\V$ if for every $x \in \Delta_m$ there is $y \in \L$ such that the following holds for all $v \in \V$ \begin{align}\label{eq:epsnet_val} |v \cdot x - v\cdot y| \leq  \eps v \cdot x\end{align} Moreover, we say the net is \emph{effective} if there is an algorithm which takes as input $x \in \Delta_m$ and outputs $y \in \L$ satisfying \eqref{eq:epsnet_val} in time $\poly(m)$
\end{definition}

\begin{lemma}\label{lem:lottery_to_menu_net1}
  If $\L$ is an $\epsilon^2$-net of $\Delta_m$ with respect to $\V \sse [1,H]^m$, and $\M$ is a family of menus, then there is a one-sided $?\eps$-net  $\N$ of $\M$ with respect to $\V$ witn $|\N| \leq ?? \frac{1}{\eps^2}^{|\L|}$. Moreover, if $\L$ is effective, then so is $\N$. 
\end{lemma}
\begin{proof}

For each $M \in \M$, include in $\N$ an approximation $\tilde{M}$ of $M$, defined as follows. For every $(x,p)$ in $M$, include in $\tilde{M}$ the entry  $(\tilde{x},\tilde{p})$ defined as follows
\begin{itemize}
\item $\tilde{p} = (1-\eps^2)^t$ is the greatest integer power of $(1-\eps^2)$ not exceeding $p$
\item $\tilde{x} = (1-\eps) y (1+\eps^2)^t$
%\item $\tilde{x} \in \L$ and $|v \cdot x - v \cdot \tilde{x} | \leq \eps^2 v \cdot x$ for every $v \in \V$ 
%\item Let $(1-\eps^2)^t$ be the result of rounding down $p$ to the nearest integer power of  $1- \eps^2$, and let $\tilde{p}= (1-\eps^2 - \eps^3)^t $
\end{itemize}

We now claim that $\Rev(M, v) - \Rev(\tilde{M},v) \leq 6 \eps$ for every $v \in \V$. Intuitively,  the mapping $(x,p) \to (\tilde{x},\tilde{p})$ described above changes a player's value for allocation $x$ by at most $\eps^2$, and reduces the price $p$ by a quantity between $\eps^2$ and $ \eps+\eps^2$ which increases as $p$ increases. This increasing discount for pricy lotteries makes them comparatively more attractive, limiting the decrease in revenue. Formally, for $(x,p) \in M$, we can bound the change of utility  $(v \cdot \tilde{x} - \tilde{p}) - (v \cdot x - p)$ as follows.
\begin{align*}
  p\eps + 2 \eps^2 \geq  \floor{p/\eps^2} \eps^3 + 2\eps^2  \geq (p-\tilde{p}) - (v \cdot x - v\cdot \tilde{x})  
\geq \floor{p/\eps^2} \eps^3 - \eps^2 \geq p \eps - 2 \eps^2
\end{align*}

Now assume that a buyer $v$ buys lottery $(x,p) \in M$, and $(\tilde{y},\tilde{q}) \in M'$. 
%
%
\begin{align*}
v \cdot y - q  &\leq v \cdot x - p \\ 
v \cdot \tilde{y} - \tilde{q}  &\geq v \cdot \tilde{x} - \tilde{p} \\
q\eps + 2 \eps^2 \geq (v \cdot \tilde{y} - \tilde{q}) - (v \cdot y - q)&\geq (v \cdot \tilde{x} - \tilde{p}) - ( v \cdot x - p) \geq p\eps - 2 \eps^2  \\
q\geq p - 4 \eps \\
\end{align*}

Since $\tilde{q} \geq q - \eps - \eps^2$, we conclude that $\tilde{q} \geq p - 6 \eps$, establishing that $\N$ is a one-sided $\epsilon$-net of $\M$. Moreover, since $\L$ is effective, the mapping $M \to \tilde{M}$ is proof that $\N$ is effective.
\end{proof}


\begin{lemma}\label{lem:lottery_to_menu_net2}
  If $\L$ is an $\epsilon^2$-net of $\Delta_m$ with respect to $\V \sse [0,1]^m$, then there is a one-sided $6\eps$-net  $\N \sse \M_k$ of  $\M_k$ with respect to $\V$ with $|\N| \leq ( \frac{|\L|}{\eps^2})^k$. Moreover, if $\L$ is effective, then so is $\N$. 
\end{lemma}
\begin{proof}
The net is $\N$ is constructed as in the proof of Lemma \ref{lem:lottery_to_menu_net1}. When $\M=\M_k$ it is easy to see that $|\N| \leq ( \frac{|\L|}{\eps^2})^k$.
\end{proof}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pricing"
%%% End: 


==> nets.tex <==
\section{Covers and Menu Complexity}
\label{sec:covers}


Our primary tool for bounding the complexity of pricing problems is reminiscent of $\epsilon$-covers of a metric space, though importantly different. Specifically, our positive results involve identifying a small (say, exponential) family of menus, each of which has a short description (usually, a polynomial number of menu entries), which is guaranteed to include a near optimal menu from the larger family of interest. For our applications, we use the following (strong) definition.


\begin{definition}
  Let $\N$ and $\M$ be two families of menus with $\N \sse \M$, and $\V \sse [1,H]^m$
  \footnote{For ease of presentation, we write $H$ as a constant here. Our
  techniques permit $H$ to depend on $m$.} a family of valuations.
  We say $\N$ is a \emph{one-sided $\epsilon$-cover} of $\M$ with respect to $\V$ if for every $M \in \M$ there is $N \in \N$ such that for all $v \in \V$ \begin{align}\label{eq:epscover}\Rev(N,v) \geq e^{-\eps} \Rev(M,v).\end{align} 
%We say the cover is \emph{succinct} if every $N \in \N$ has a finite number of entries, and all real numbers in $N$ are rational numbers of at most  $\poly(m, \log H, \frac{1}{\epsilon})$ bits each. A cover is  \emph{effective} if there is an algorithm  which takes as input any finite $M \in \M$ expressed in $\langle M \rangle$ bits,  and outputs $N \in \N$ with $|N| \leq |M|$ satisfying \eqref{eq:epscover} in time $\poly(\langle M \rangle,m,\frac{1}{\eps}, \log H)$. 
We say a cover is  \emph{effective} if there is an algorithm  which takes as input any finite $M \in \M$,  and outputs $N \in \N$ with $|N| \leq |M|$ satisfying \eqref{eq:epscover} in time $\poly(|M|,m,\frac{1}{\eps}, \log H)$. 
\end{definition}



We now take a moment to reflect on this definition, and its relation to the traditional notion of an $\epsilon$-cover of a metric space. In the ensuing discussion, think of $\M$ as $\M_\infty$, the family of all mechanisms, and $\N$ as a finite family of mechanisms of small description complexity. One can think of every menu (i.e. mechanism)  $M $ as a function  mapping valuations $v \in \V$ to the logarithm of the revenue generated by the auctioneer. Viewed thus, the $\ell_\infty$ metric on the resulting function space serves as a natural distance function on menus. A (2-sided) $\epsilon$-cover of the metric space of menus, if a small one exists, guarantees that a small number of samples from a distribution $\D$, presented as an oracle, suffice to estimate the expected revenue of \emph{every} menu simultaneously to within a small multiplicative error. Such a guarantee, often referred to as \emph{uniform convergence},  bounds the description complexity of an approximately optimal mechanism, as well as the sample complexity of finding such a mechanism.  To see this, observe that an optimal mechanism for the small sample is approximately optimal for the hidden distribution $\D$, with high probability. In effect, uniform convergence reduces finding the optimal mechanism for the hidden distribution to finding the optimal mechanism for the sample, in analogy to \emph{empirical risk minimization} in PAC learning. Uniform convergence guarantees are commonplace in the machine learning literature, and have even been suggested and applied to optimal mechanism design by Balcan et al \cite{balcan}. However, as we show in Appendix \ref{app:nocover}, finite $\epsilon$-covers in the classical (i.e., 2-sided) sense do not exist for the space of pricing mechanisms, even in the special case of pricing a single item. This observation motivates our weaker definition.


If a family  $\M$ of menus admits a small one-sided $\epsilon$-cover $\N$ with respect to $\V$, and $\D$ is supported on $\V$, we can still bound the number of samples necessary to identify a near optimal menu in $\M$. Specifically, using well-known concentration inequalities and the union bound, we conclude that $\log |\N|$ samples from $\D$ suffice for approximately estimating  $\Rev(N,\D)$ for every $N \in \N$. Whereas we can not make such a guarantee for every menu $M \in \M$ in the larger class, we do not need to, since  some $N \in \N$ is approximately optimal! There is one quirk of this approach, due to the fact that our $\epsilon$-cover is one sided: it no longer suffices to output the revenue-maximizing menu in $\M$ using the sampled valuations, as such a menu may not lie in $\N$, and may therefore have revenue that differs substantially from that estimated by our sample. Our algorithm must in fact output a menu in the cover $\N$ to avoid \emph{over-fitting} to the sample.\footnote{Our technique of fitting an element of a small cover of all menus can be thought of as a discrete variant of \emph{regularization}, a technique thoroughly employed in the machine learning community.} This is OK for bounds on the sample and description complexity, but introduces a computational challenge for our applications: when $\M=\M_\infty$ is the space of all menus, finding an optimal unconstrained menu for an explicitly given distribution (the sample) reduces to solving a simple linear program. The same cannot be said of the finite covers $\N$ we construct. Fortunately, we show below that it suffices to exhibit an efficient ``rounding procedure'' which maps menus in $\M$ to menus in $\N$, as doing so recovers computational tractability. We summarize these observations in Algorithm \ref{alg:main} and Lemma \ref{lem:alg}.


\begin{algorithm}
\caption{Sample \& Round Pricing Algorithm}
\label{alg:main}
\begin{algorithmic}[1]
  \PARAMETER Family $\V \sse [1,H]^m$ of valuations
  \PARAMETER Family $\M$ of menus
  \PARAMETER An $\epsilon$-cover $\N$ of $\M$ with respect to $\V$
  \INPUT Distribution $\D$ with support $\V$, presented as a black box
  \OUTPUT $N \in \N$ satisfying $\Rev(N,\D) \geq (1-3\eps) \Rev(M,\D)$ for every $M \in \M$, w.h.p
  \STATE Sample $n = \poly(m, H, \log |\N|, \frac{1}{\eps})$ times from $\D$,
  denote the samples by $S = \{ v_1, \cdots, v_n \}$;
  \STATE Let $M_S\in \argmax_{M \in \M} \Rev(M,S)$ 
  \STATE Let $N_S \in \N$ satisfy $\Rev(N_S,v) \geq e^{-\eps} \Rev(M_S,v) $ for every $v \in \V$ (Equation \eqref{eq:epscover})
  \STATE Output $N_S$
  \end{algorithmic}
\end{algorithm}


\begin{lemma}\label{lem:alg}
  If $\N$ is a one-sided $\epsilon$-cover of $\M$ with respect to $\V \sse
  [1, H]^m$, and $\Rev(\M,\D) \geq 1$,\footnote{This requirement that the revenue of the optimal menu is not too small serves to rule out trivial menu families, which are not of interest to us, and consequently simplify our guarantees.} then Algorithm \ref{alg:main} outputs $N \in \N$ such that $\Rev(N,\D) \geq (1-3\eps) \Rev(\M,\D) $, with high probability. Moreover, when $\M=\M_\infty$ and $\N$ is an effective cover, Algorithm \ref{alg:main} runs in $\poly(m, H, \log |\N|, \frac{1}{\eps})$ time.
\end{lemma}
\begin{proof}
We begin by showing that the sample $S$ provides an estimate, within an additive $\epsilon$, of the revenue of every menu $N \in \N$.  For any fixed $N \in \N$, by the Hoeffding bound we have $Pr[|\Rev(N, \D) - \Rev(N,S)| > \eps] \le 2e^{-\frac{2n \eps^2}{H^2}}$. Applying the union bound, we get 
  \begin{equation}
  Pr[\exists N \in \N \text{ s.t. } |\Rev(N, \D) - \Rev(N,S)| > \eps] \le 2
  e^{-\frac{2n \eps^2}{H^2}} |\N|
  \end{equation}
  So when the number of samples $n$ is  $poly(m, H, \frac{1}{\eps}, \log |\N|)$, the empirical revenue of every menu in $\N$ approximates its revenue on $\D$ to within an additive $\epsilon$ with high probability.
  

Let $M^*$ be an optimal menu for distribution $\D$. Using the Hoeffding bound again, we conclude that $|\Rev(M^*, S) - \Rev(M^*, \D )| \leq \epsilon$ with high probability --- i.e. the empirical revenue of $M^*$ approximates its revenue on $\D$ to within an additive $\epsilon$. The following holds with high probability, completing the proof of the approximation guarantee.
\begin{align*}
  \Rev(N_S, \D) &\geq \Rev(N_s,S) - \eps \\
  &\geq e^{-\eps} \Rev(M_s, S) - \eps \\
  &\geq e^{-\eps} \Rev(M^*,S) -\eps \\
  &\geq e^{-\eps} \Rev(M^*,\D) - 2\eps \\
&\geq (1-3\eps) \Rev(M^*,\D)
\end{align*}


We now analyze the runtime of this algorithm when $\M=\M_\infty$ and $\N$ is effective.  Recall that step 2 reduces to solving a linear program with $O(nm)$ variables, and outputs a menu $M_S$ with $|M_S| \leq n$. Step 3 then runs in $\poly(n,m)$ time, since $\N$ is effective. 
  \end{proof}
Algorithm \ref{alg:main}  and Lemma \ref{lem:alg} reduce the task of bounding the (descriptive, sample, and computational) complexity of pricing problems to the design of  one-sided $\epsilon$-covers.
Our main technique for constructing one-sided $\epsilon$-covers  is through constructing a two-sided cover of the set of lotteries, defined below.

\begin{definition}
  A family $\L \sse \Delta_m$ of lotteries is a (two-sided) $\sigma$-cover of $\Delta_m$ with respect to $\V \sse [1,H]^m$ if for every $x \in \Delta_m$ there is $y \in \L$ such that the following holds for all $v \in \V$ 
%
\begin{align}\label{eq:epscover_lottery} e^{-\sigma} v \cdot y  - \sigma \leq v \cdot x \leq e^\sigma v \cdot y + \sigma \end{align} 
%
%\begin{align}\label{eq:epscover_lottery} \frac{v \cdot x}{ v\cdot y} \in [e^{-\eps},e^{\eps}]\end{align} 
%
%We say the cover is \emph{succinct} if $|\L|$ is finite, and moreover every $x \in \L$ is a rational vector with  $\poly(m, \log H, \frac{1}{\eps})$ bits. We say a succinct cover is \emph{effective} if there is an algorithm which takes as input $x \in \Delta_m$, with rational entries totalling  $\langle x \rangle$ bits,  and outputs $y \in \L$ satisfying \eqref{eq:epscover_lottery} in time $\poly(\langle x \rangle, m,\log H, \frac{1}{\eps})$
We say a cover is \emph{effective} if there is an algorithm which takes as input $x \in \Delta_m$,  and outputs $y \in \L$ satisfying \eqref{eq:epscover_lottery} in time $\poly( m,\log H, \frac{1}{\sigma})$

\end{definition}




\begin{lemma}\label{lem:lottery_to_menu_cover}
Fix $\epsilon >0$ and $k \in \NN \union \set{\infty}$. 
  If $\L$ is an $\frac{\epsilon^2}{\log H}$-cover of $\Delta_m$ with respect to $\V \sse
  [1,H]^m$, then there is a one-sided $8\eps$-cover
  $\N$ of $\M_k$ with respect to $\V$ with $|\N| \leq  \min\left\{\left(\frac{\log H}{\eps}\right)^{2|\L|},  \left(\frac{ \log^2 H |\L|}{\eps^2}\right)^k \right\}$ and $\N \sse \M_{|\L|}$. 
%  If $\L$ succinct then so is $\N$, and if $\L$ is effective then so is $\N$.
Moreover, if $\L$ is effective then so is $\N$.
\end{lemma}
\noindent We note that when $k=\infty$, the guarantee on the size of $\N$ simplifies to $\left(\frac{\log H}{\eps}\right)^{2|\L|}$. 

%We relegate the highly technical proof of Lemma \ref{lem:lottery_to_menu_cover} to Appendix \ref{app:covers}.

\begin{proof}
Denote $\sigma = \frac{\epsilon^2}{\log H}$. We define for every (non-zero) allocation/price pair $(x,p)$ a rounded version $(\tilde{x},\tilde{p}) = r(x,p)$, as follows:
\begin{itemize}
\item Let $ p' = e^{t\sigma}$ be the result of rounding $p$ down to the nearest integer power of $e^\sigma$. Note that $t(p) \in \set{0,1,\ldots,\left\lfloor{\frac{\log H}{\sigma}}\right\rfloor}$
\item Let $x' \in \L$ satisfy $e^{-\sigma} v \cdot x - \sigma \leq v \cdot x' \leq e^\sigma v \cdot x + \sigma$  for every $v \in \V$. (Equation \eqref{eq:epscover_lottery})
\item Define the ``bonus'' multiplier $b=b(p)=  e^{t \sigma^2/\eps }$. Note that $b(p) \in [1, e^{\eps}]$ is nondecreasing in $p$.
\item Define the ``discount'' $d=d(p) = t \frac{\sigma^2}{\eps}$. Note that $d(p) \in [0,\eps]$.
\item Let $\tilde{p} = e^{- \eps}  \cdot p' / b - d$, and $\tilde{x} = e^{-\eps} \cdot b \cdot x'$. 
%\item Let $\tilde{x} =  e^{t  \sigma^2 / \eps - \eps} x'$. Note that $ e^{-\eps} x' \leq \tilde{x} \leq x'$ component-wise.
\end{itemize}
We naturally extend this definition to menus. For each menu $M$, we let $\tilde{M} = \set{r(x,p): (x,p) \in M}$. Finally, we define our net $\N$ as the set of all rounded menus from $\M$, i.e. $\N = \set{\tilde{M} : M \in \M}$. 
 %It is easy to see that $\N$ is succinct when $\L$ is succinct, and $\N$ is effective when $\L$ is effective.
By examining the map $M \to \tilde{M}$, it is easy to see that $\N$ is effective when $\L$ is effective.

Note that rounded allocation/price pairs $(\tilde{x},\tilde{p})$ are in one to one correspondance with $\L \cross \set{0,1,\ldots,\left\lfloor{\frac{\log^2 H}{\eps^2}}\right\rfloor}$. Since, without loss of generality, every lottery appears at most once in any menu $N \in \N$, we have that $N \sse \M_{|\L|}$ and  $|\N| \leq \left(\frac{\log H}{\eps}\right)^{2|\L|}$.  Moreover, since every $N \in \N$ has at most $k$ entries, each of which is a rounded allocation/price pair, we have that $|\N| \leq \left(\frac{ \log^2 H |\L|}{\eps^2}\right)^k$.


We now claim that $\Rev(M, v) \geq e^{-8\eps} \Rev(\tilde{M},v)$ for every $v \in \V$.  Intuitively,  the mapping $r: (x,p) \to  (\tilde{x},\tilde{p})$ can be thought of as the composition of two mappings: $(x,p) \to (x',p')$ and $(x',p') \to (\tilde{x},\tilde{p})$. The former introduces error into each of $v \cdot x$ and $p$, which may have the undesirable consequence of changing a player's choice and thus reducing the auctioneer's
 revenue on $v$. The purpose of the latter mapping is to fix this by providing a bonus/discount for pricy lotteries in order to make them comparatively more attractive.

Formally, assume for a contradiction that $\Rev(M, v) < e^{-8\eps} \Rev(\tilde{M},v)$ for some $v \in \V$. Let $(x,p)$ be the chosen allocation/price pair from menu $M$, and $(\tilde{y},\tilde{q}) = r(y,q)$ be the chosen pair from menu $\tilde{M}$.  Denoting $(\tilde{x},\tilde{p}) = r(x,p)$, it follows that

\begin{align}
(v \cdot x - v \cdot y)  - (p - q) &\geq 0  & &\mbox{(By the choice of $(x,p)$ from $M$)} \label{eq:pq}\\
(v \cdot \tilde{x} - v \cdot \tilde{y})  - (\tilde{p} - \tilde{q}) &\leq 0 & &\mbox{(By the choice of $(\tilde{y},\tilde{q})$ from $\tilde{M}$)} \label{eq:pqtilde}
\end{align}

\noindent Moreover, $p$ is significantly larger than $q$.

\begin{align}\label{eq:bonuspq}
p &> e^{8 \eps} \tilde{q} \notag &&\mbox{(By assumption)} \\
&= e^{7 \eps}  q' / b(q) - d(q) \notag &&\mbox{(By definition of $r(.)$)} \\ 
&\geq e^{6 \eps} q'  - \eps  \notag  &&\mbox{(Since $b(q) \leq e^\eps$ and $d(q) \leq \eps$)} \\
&\geq e^{6 \eps - \sigma} q - \eps \notag &&\mbox{(Since $q' \geq e^{-\sigma} q$, by definition)}  \\ 
& \geq e^{5 \eps} q - \eps \notag &&\mbox{(Since $\sigma \leq \eps$)}  \\
& \geq e^{4 \eps} q.  & & \mbox{(Since prices are at least 1 (see Section \ref{sec:prelim}))}
\end{align}


Inequality \eqref{eq:bonuspq} and the definition of $r(.)$ imply that $t(p) - t(q) \geq  \frac{4 \eps}{\delta}$, and therefore that $\frac{b(p)}{b(q)} \geq e^{\frac{4 \eps}{\delta} \frac{\delta^2}{\eps}}= e^{4\sigma} $ and $d(p) - d(q) \geq \frac{4 \eps}{\delta} \frac{\delta^2}{\eps} = 4 \sigma$; i.e. the larger price is given a substantially larger bonus and discount. Using this fact, we reach a contradiction with \eqref{eq:pq} and \eqref{eq:pqtilde}, completing the proof.


% \begin{claim}
%   Assume $(x,p)$ and $(y,q)$ are such that $q < p - \eps$. It is the case that $\tilde{p} - \tilde{q} \leq e^{-\eps} (p- q)$.
% \end{claim}
% \begin{proof}
  \begin{align}
    \tilde{p} - \tilde{q} &= e^{- \eps} ( p' / b(p) -  q' / b(q)) - (d(p) - d(q) &  \mbox{(By definition of  $r(.)$)} \notag\ \\
 & \leq e^{- \eps} (  p / b(p) - q e^{-\sigma} / b(q)     )  - (d(p) - d(q)) & \mbox{(Since $p' \leq p$ and $q' \geq e^{-\sigma} q$)} \notag\\
&\leq e^{- \eps} (  p / b(p) - q  / b(p)  ) - 4 \sigma & \mbox{(Since $b(p) \geq e^\sigma b(q)$ and $d(p) - d(q) \geq 4 \sigma$)} \notag\\
&\leq e^{- \eps} ( p - q ) -4\sigma & \mbox{(Since $b(p) \geq 1$)} \notag \\
&< e^{- \eps} ( p - q ) -3\sigma & 
  \end{align}
%\end{proof}


%\begin{claim}
%  Assume $(x,p)$ and $(y,q)$ are such that $q < p - 2\eps$. It is the case that $v\cdot \tilde{x} - v \cdot \tilde{y} \geq e^{-\eps} (v \cdot x-  v \cdot y)$.
%\end{claim}
%\begin{proof}
  \begin{align}
    v\cdot \tilde{x} - v \cdot \tilde{y} &= e^{-\eps}[ b(p) \cdot  v  \cdot  x'  - b(q) \cdot v  \cdot  y'  ] & \mbox{(By definition of  $r(.)$)} \notag\\
    &\geq e^{-\eps}[ b(p) (  e^{-\sigma} v  \cdot  x - \sigma)  - b(q) (e^\sigma v  \cdot  y + \sigma ) ] & \mbox{(By definition of  $r(.)$)} \notag\\
    &= e^{-\eps}( e^{-\sigma} b(p)    v  \cdot  x   -  e^\sigma  b(q) v  \cdot  y )  - e^{-\eps} (b(p) + b(q)) \sigma &  \notag\\
    &\geq e^{-\eps}( e^{-\sigma} b(p)    v  \cdot  x   -  e^\sigma  b(q) v  \cdot  y )  - 2 \sigma &  \mbox{(Since $b(p), b(q) \leq e^\eps $)} \notag\\
     &\geq e^{-\eps}(  e^{\sigma} b(q)  \cdot v \cdot x  - e^\sigma b(q)  \cdot v \cdot   y  ) - 2 \sigma &\mbox{(Since $b(p) \geq e^{2\sigma} b(q)$)} \notag\\
&\geq e^{-\eps}( v \cdot x  - v \cdot   y  ) - 2 \sigma & \mbox{(Since $e^\sigma b(q) \geq 1$)} \notag\\
&> e^{-\eps}( v \cdot x  - v \cdot   y  ) - 3 \sigma & 
  \end{align}
%\end{proof}
\end{proof}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pricing"
%%% End: 


==> nocover.tex <==
\section{A Note on Covers and Uniform Convergence}
\label{app:nocover}
We now justify our use of one-sided $\epsilon$-covers as a ``regularized'' family of mechanisms from which we select. We would have liked to instead use a $2$-sided $\epsilon$-cover $\N$ of the family of $C$-menus, as the existence of such an object would lead to a \emph{uniform convergence} result: sampling $\poly(\log |\N|)$ times from our distribution suffices to estimate the revenue of \emph{every} menu of size $C$, and the ``obvious'' algorithm which simply selects the optimal such menu for the sample is approximately optimal.

Unfortunately this is not the case, and we can not rule out ``over-fitting'' by the obvious algorithm to the sample. In fact, a $2$-sided $\epsilon$-cover does not exist even in the special case of a single item auction. Consider the family of deterministic auctions of a single item, each of who's menu contains a single entry of the form $(1,p)$. It is easy to verify that no single mechanism approximates the revenue of two different determinstic auctions with prices $p_1, p_2 \in [H/2, H]$ --- any such mechanism must err by at least $\min(p_1,p_2)> H/2$ on inputs between $p_1$ and $p_2$. Therefore, any $2$-sided $\epsilon$-cover must be infinite.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pricing"
%%% End: 


==> radermacher.tex <==
\section{The Radermacher Complexity of Pricing}
\label{sec:radermacher}
% Given a discretization parameter $\epsilon$, the total number of possible price
% vectors is
% \begin{equation}
% T = (\frac{L}{\epsilon})^n
% \end{equation}
% Denote them by $p_1, p_2, \cdots, p_T$.


We will use $m$ to denote the number of items, $n$ to
denote number of samples. To simplify notation:
\begin{definition}
Given menu $L$, the associated revenue function $f[L]: R^m \rightarrow R$ is
defined as:
\begin{equation}
f[L](v) = (\argmax_{(x, r) \in L} \{ \vec{v} \cdot x - r\}) \cdot (0, 1)
\footnote{We assume that the buyer would break ties by choosing the most
expensive lottery}.
\end{equation}

Let $\mathcal{F}$ be the set of all possible revenue functions, i.e.
$\mathcal{F} = \{ f[L]: L \text{ is a lottery} \}$.
\end{definition}

\begin{definition}[Sample Average]
Given sample $S = (\vec{v}_1, \cdots, \vec{v}_n)$ and lottery $L$,
sample average of function $f[L]$ is defined as 
\begin{equation}
\hat{E}_S[f[L]] :=\frac{1}{n}
\sum_{i=1}^n f[L](\vec{v}_i).
\end{equation}
\end{definition}

\begin{definition}
Sample $S = (\vec{v}_1, \cdots, \vec{v}_n)$ (where valuation vector $\vec{v}_i
\in R^m$ for all $i$) is an $\epsilon$-good sample for lottery $L$ (or
equivalently its induced revenue function $f[L]$) if 
\[
|
\hat{E}_S[f[L]] - E_{\vec{v} \sim X}[f[L](\vec{v})] 
| 
\le \epsilon
\]
\end{definition}

A natural idea is trying to prove that w.h.p. $S$ is a good sample
for all possible revenue functions. Note that if the space of all revenue
function can be cover by an $\eps$-net of exponential size, then \textit{Union
Bound} works.
But the space of all lottery revenue functions is doubly exponential
\footnote{
Roughly, $\frac{nL}{\epsilon}^{(\frac{1}{\epsilon})^n}$, while the number for
item pricing is $(\frac{L}{\epsilon})^n$}.

% First, instead of aiming at either multiplicative approximations or additive
% approximations. We use Partial-Multiplicative Approximation (PMA) \footnote{I
% coined this term myself, feel free to change it. I regard it as a combination
% of multiplicative and additive bounds}.
% 
% \begin{definition}
% An algorithm $A$ is an $(\sigma, \alpha)$-PMA if for any instance $I$:
% \begin{enumerate}
%   \item When $OPT(I) \le \sigma$, $0 \le A(I) \le \sigma$
%   \item When $OPT(I) > \sigma$, $A(I) \ge \frac{OPT(I)}{\alpha}$
% \end{enumerate}
% \end{definition}
% 
% The point of this definition is that when $OPT$ is very small ($\le \sigma$),
% then we no longer require algorithm $A$ to produce a multiplicatively close
% solution. Another way to look at this is: \textit{Promise Problem}.

\subsection{Rademacher Complexity and Uniform Convergence}
\begin{definition}[Rademacher Complexity]
Let $S = (v_1, v_2, \cdots, v_n)$ be $n$ independent samples from valuation
distribution $D$, i.e. $v_i \sim D$.
The empirical Rademacher complexity of $\mathcal{F}$ on $S$ is defined as:
\begin{equation}
\hat{R}(\mathcal{F}, S) = \frac{1}{n} E_{\lambda}[\sup_{f \in
\mathcal{F}} \{ \sum_{i=1}^n \lambda_i f(v_i) \}]
\end{equation}
where $\lambda_i$ are i.i.d symmetric Bernoulli variables.
The worst-case Rademacher complexity of $\mathcal{F}$ is
defined as:
\begin{equation}
\sup_{S \in X^n} \hat{R}(\mathcal{F}, v) \footnote{We abuse notation by using X
also as the support of X}
\end{equation}

The expected Rademacher complexity of $\mathcal{F}$ with respect to distribution
$X$ is defined as:
\begin{equation}
R_k(\mathcal{F}, X) = E_{S \sim X^k} [\hat{R}(\mathcal{F}, S)]
\end{equation}
We abbreviate $R_k(\mathcal{F}, X)$ as $R_k(\mathcal{F})$ when the context is
clear.
\end{definition}

\begin{thm}
For $0 < \delta < 1$, and sample set $S = (v_1, \cdots, v_K)$. With probability
$1 - \delta$ (over the randomness of sampling): for every function $f: R^m
\rightarrow [0, m \cdot L]$ in $\mathcal{F}$,
\begin{equation}
\hat{E}_S[f(v)] \le E_{v \sim X}[f(v)] + 2R_k(\mathcal{F}) +
3\sqrt{\frac{\ln(\frac{2}{\delta})m^2L^2}{K}}
\end{equation}
\end{thm}

So this means that if the Rademacher complexity is small, then with high
probability sample $S$ will be a good sample for every function $f$ in
$\mathcal{F}$, provided $K$ is sufficiently large.

As long as we allow the sample complexity be polynomial in $L$ and $K$, the last
term can be negligible. And in the hope that $R_k(\mathcal{F})$ also decreases
polynomially in $K$ and $L$, the second term can also be negligible. 
Then using only polynomially many samples, we can with high probability achieve: 
\begin{equation}
\hat{E}_S[f(v)] \le E_{v \sim X}[f(v)] 
+ o(1), \forall f \in \mathcal{F}
\end{equation}
% As we also have $f(L^\ast_V, S) \ge f(L^\ast_X, S)$ and $f(L^\ast_X, S) \ge (1 - \epsilon) f(L^\ast_X,
% X)$ with high prob.:
% \begin{equation}
% f(L^\ast_V, X) =E_{v \sim X}[f[L^\ast_V](v)] \ge
% \hat{E}_S[f[L^\ast_V](v)] - o(1) 
% \end{equation}
% \begin{equation}
% \ge f(L^\ast_X, S) - o(1) \ge (1 - \epsilon) (f(L^\ast_X,
% X) - o(1))
% \end{equation}

% So now we need to bound $\hat{R}_m(\mathcal{F})$ or
% \begin{equation}
% E_{S,\bar{S}}[\sup_{f \in \mathcal{F}} \{ \hat{E}_S[f] -
% \hat{E}_{\bar{S}}[f] \}]
% \end{equation}
% \begin{equation}
% =\frac{1}{m} E_{S,\bar{S}}[\sup_{f \in \mathcal{F}} \sum_i (f(v_i) -
% f(\bar{v_i}))]
% \end{equation}
% 
% \begin{align*}
% \exp(t \cdot E_{S,\bar{S}}[\sup_{f \in \mathcal{F}} \sum_i (f(v_i) -
% f(\bar{v_i}))])
% \\ \le E_{S,\bar{S}}[\exp(t \cdot \sup_{f \in \mathcal{F}} \sum_i
% (f(v_i) - f(\bar{v_i})))] 
% \\ = E_{S,\bar{S}}[\sup_{f \in \mathcal{F}} \exp(t \sum_i (f(v_i) -
% f(\bar{v_i})))] 
% \\ \le \sum_{f \in \mathcal{F}} E_{S,\bar{S}}[\exp(t \sum_i (f(v_i) -
% f(\bar{v_i})))] 
% \\ = \sum_{f \in \mathcal{F}} \prod_{i=1}^m E_{S,\bar{S}}[\exp(t \cdot (f(v_i) -
% f(\bar{v_i})))]
% \\ = \sum_{f \in \mathcal{F}} (E_{v \sim S, v \sim \bar{S}}[\exp(t \cdot (f(v) -
% f(\bar{v})))])^m
% \end{align*}



% \subsection{2 Different definition of Covering Number}
% \begin{definition}[Shaddin's]
% \label{shaddin_def}
% Given two functions $f$ and $g$,
% define metric $d(f, g) = \sup_{\vec{v} \in X} \{f(\vec{v}) - g(\vec{v})\}$.
% \footnote{$X$ is the valuation distribution, I am abusing notation here.}
% Then the $\epsilon$-covering number of function class $\mathcal{F}$ is the
% minimum number of functions (not necessarily in $\mathcal{F}$) whose
% $\epsilon$-balls together cover the function class $\mathcal{F}$.
% \end{definition}
% 
% \begin{definition}[Standard ML]
% Given function class $\mathcal{F}$,
% $n$ samples $S = \{\vec{v_1}, \cdots, \vec{v_n}\}$ where $\vec{v_i} \in X
% \subset R^m$ \footnote{m = \#item, abusing notation of $X$ again here.}, the
% (empirical) covering number $\mathcal{N}_{\infty}(\mathcal{F}, \epsilon, S)$ is defined as the minimum number $c$ of vectors $r_1, r_2, \cdots, r_c \in R^n$ such that
% for any $f \in \mathcal{F}$, there exists $r_i$ such that $|(f(v_1), f(v_2),
% \cdots, f(v_n)) - r_i|_{\infty} \le \epsilon$.
% Then define $\mathcal{N}_{\infty}(\mathcal{F}, \epsilon, n) = \sup_{S:|S|=n}
% \mathcal{N}_{\infty}(\mathcal{F}, \epsilon, S)$.
% \end{definition}
% \begin{remark}
% Note that the covering number here is defined with respect to a sample
% size $n$. If we let $n$ be the cardinality of $X$ (possibly uncountably
% infinite), then these two definitions coincide.
% \end{remark}
% 
% Pollard proved that 
% \begin{thm}
% \begin{equation}
% Pr_{S \sim X^n}[\sup_{f \in \mathcal{F}} \{ \hat{E}_S[f] - E[f] \} >
% \epsilon] \le c \: \mathcal{N}_{1}(\mathcal{F}, \frac{\epsilon}{8}, n)
% \exp(O(\frac{-n \epsilon^2}{L^2}))
% \end{equation}
% \end{thm}
% So Definition \ref{shaddin_def} seems to be too strong here if $\mathcal{N}$ is
% monotone w.r.t. $n$.

% \subsection{Rademacher complexity of single-dimension functions}
% We are interested inthe Rademacher complexity of the following class of
% functions:
% \begin{equation}
% \mathcal{F} = \{ f: X \rightarrow R: \| f \| \le B \} 
% \end{equation}
% If we assume that all the $f$ are lipschitz continuous, then we can discretize
% domain $X$ into levels: $\{l_0, l_1, \cdots, l_t\}$.
% And then WLOG assuming $x = l_i$:
% \begin{equation}
% f(x) \approx \inprod{(f(l_0), f(l_1), \cdots, f(l_t)), e_i }
% \end{equation}
% \begin{align*}
% \mathcal{R}_S(\mathcal{F}) &= \frac{2}{m} E_{\sigma} \max_{f \in \mathcal{F}}
% \sum_{i=1}^m \sigma_i f(x_i) \\
% &= \frac{2}{m} E_{\sigma} \max_{ \norm{w} \le B} \sum_{i=1}^m \sigma_i
% \inprod{w, e_{x_i}}
% \\
% &\approx \frac{2}{m} E_{\sigma} \max_{ \norm{w} \le B}  \inprod{w,
% \sum_{i=1}^m \sigma_i e_{x_i}}
% \\
% &= \frac{2}{m} E_{\sigma} \max_{ \norm{w} \le B}  \norm{w}
% \norm{\sum_{i=1}^m \sigma_i e_{x_i}}
% \\
% & \le \frac{2B}{m} E_{\sigma} \norm{ \sum_i \sigma_i
% e_{x_i}}
% \\
% & \le \frac{2B}{m} E_{\sigma} 
% \sqrt{\inprod{\sum_i \sigma_i e_{x_i}, \sum_i \sigma_i e_{x_i}}}
% \\
% & \le \frac{2B}{m}  
% \sqrt{E_{\sigma} \inprod{\sum_i \sigma_i e_{x_i}, \sum_i \sigma_i e_{x_i}}}
% \\
% & \le \frac{2B}{m}  
% \sqrt{E_{\sigma} \sum_i \sum_j \sigma_i \sigma_j \inprod{e_{x_i}, e_{x_j}}}
% \\
% & \le \frac{2B}{m}  
% \sqrt{ \sum_i \sum_j E_{\sigma} [\sigma_i \sigma_j] \inprod{e_{x_i}, e_{x_j}}}
% \\
% & \le \frac{2B}{m}  
% \sqrt{ \sum_i \inprod{e_{x_i}, e_{x_i}}}
% \\
% & \le \frac{2B}{m}  
% \sqrt{ \sum_i \inprod{e_{x_i}, e_{x_i}}} = \frac{2B}{m} \sqrt{m} = \frac{2B}{\sqrt{m}}
% \end{align*}
% 
% If we restrict $f$ to be a lipschitz monotone function that satifies:
% \begin{enumerate} 
%   \item $0 \le f(x') - f(x) \le x' -x$ for $x' \ge x$;
%   \item $f(0) = 0$;
%   \item Supported on $[0, L]$;
% \end{enumerate}
% 
% \begin{lemma}
% If $f$ is discretized into $\{(l_0, f(l_0)), (l_1, f(l_1)), \cdots, (l_{L/\eps},
% f(l_{L / \eps})) \}$ where $l_i = \eps \cdot i$.
% Let $w_i = f(l_{i}) - f(l_{i-1})$,
% then $f(l_i) = \sum_{j=1}^i w_j = \inprod{w, (1, 1, 1, \cdots, i^{th} 1,
% 0, 0, \cdots)}$.
% Given any $x \in [0, L]$, denote by $\bar{x}$ the closest multiple of $\eps$ to
% $x$. So $\abs{f(x) - f(\bar{x})} \le \abs{x - \bar{x}} \le \eps$
% \end{lemma}
% 
% Let $S = \{ x_1, x_2, \cdots, x_n \}$ be a set of $n$ samples from $X$.
% 
% \begin{align*}
% \hat{\mathcal{R}}_S(\mathcal{F}) &= \frac{2}{n} E_{\sigma} [ \max_{f \in
% \mathcal{F}} \sum_{i=1}^n \sigma_i f(x_i) ] \\
% &= \frac{2}{n} E_{\sigma} [ \max_{ \norm{w} \le \sqrt{L \epsilon}} \sum_{i=1}^n
% \sigma_i
% \inprod{w, s_{x_i}} ]
% \\
% &\approx \frac{2}{n} E_{\sigma} [\max_{ \norm{w} \le \sqrt{L \epsilon}} 
% \inprod{w, \sum_{i=1}^n \sigma_i s_{x_i}} ]
% \\
% & \le \frac{2}{n} E_{\sigma} [ \max_{ \norm{w} \le \sqrt{L \epsilon}}  \norm{w}
% \norm{\sum_{i=1}^n \sigma_i s_{x_i}} ]
% \\
% & \le \frac{2 \sqrt{L \epsilon}}{n} E_{\sigma} \norm{ \sum_i \sigma_i
% s_{x_i}}
% \\
% & \le \frac{2 \sqrt{L \epsilon}}{n} E_{\sigma} 
% \sqrt{\inprod{\sum_i \sigma_i s_{x_i}, \sum_i \sigma_i s_{x_i}}}
% \\
% & \le \frac{2 \sqrt{L \epsilon}}{n}  
% \sqrt{E_{\sigma} \inprod{\sum_i \sigma_i s_{x_i}, \sum_i \sigma_i s_{x_i}}}
% \\
% & \le \frac{2 \sqrt{L \epsilon}}{n}  
% \sqrt{E_{\sigma} \sum_i \sum_j \sigma_i \sigma_j \inprod{s_{x_i}, s_{x_j}}}
% \\
% & \le \frac{2 \sqrt{L \epsilon}}{n}  
% \sqrt{ \sum_i \sum_j E_{\sigma} [\sigma_i \sigma_j] \inprod{s_{x_i}, s_{x_j}}}
% \\
% & \le \frac{2 \sqrt{L \epsilon}}{n}  
% \sqrt{ \sum_i \inprod{s_{x_i}, s_{x_i}}}
% \\
% & \le \frac{2 \sqrt{L \epsilon}}{n}  
% \sqrt{ \sum_i \inprod{s_{x_i}, s_{x_i}}} = \frac{2 \sqrt{L \epsilon} }{n}
% \sqrt{n \frac{L}{\epsilon}} =
% \frac{2 L}{\sqrt{n}}
% \end{align*}

% \subsection{Another bound on Rademacher Complexity}
% We have the following theorem from \cite{Kakade}:
% \begin{thm}
% Let $S$ be a convex subset in $S^d$.
% Let $\frac{1}{p} + \frac{1}{q} = 1$.
% Let $\mathcal{F}_{\mathcal{W}} = \{ x \mapsto \inprod{w, x} : w \in
% \mathcal{W} \}$. Let $\mathcal{W} = \{ w \in S : \norm{w}_q \le C \}$.
% Let $B = \sup_{x \in X} \norm{x}_p$.
% Then \begin{equation}
% \mathcal{R}_n(\mathcal{F}_{\mathcal{W}}) = B \cdot C \cdot
% \sqrt{\frac{p-1}{n}}
% \end{equation}
% \end{thm}
% 
% Note that we can express a lipschitz-continuous monotone function $f：[0, L]^m
% \rightarrow [0, mL]$ as the following:
% \begin{enumerate}
%   \item Discretize the domain $[0, L]^m$ into a $\eps$-grid $G$ of size
%   $(\frac{L}{\eps})^m$, let $d = (\frac{L}{\eps})^m$;
%   \item Let $w_1(k \cdot \eps) = f(k \cdot \eps, 0, \cdots, 0) - f((k-1)\eps,
%   0, \cdots, 0)$ \newline 
%   		Let $w_i(k_1 \cdot \eps, \cdots, k_i \cdot \eps) = f(k_1 \cdot \eps,
%   		\cdots, k_i \cdot \eps, 0, \cdots, 0) - f(k_1 \cdot \eps, \cdots,  (k_i - 1)
%   		\eps, 0, \cdots, 0)$. By lipschitz continuity, we know that $\abs{w_i} \le
%   		\eps, \forall i$.
%   \item Given a point $(k_1, k_2, \cdots, k_m)$ in $G$ (maps back into $(k_1
%   \cdot \eps, k_2 \cdot \eps, \cdots, k_m \cdot \eps) \in [0, L]^m$). Then
%   		\begin{align*}
%   		f(k_1 \eps, \cdots, k_m \eps) &= f(k_1 \eps, \cdots, k_m \eps) - f(k_1
%   		\eps, \cdots, k_{m-1} \eps, 0) \\
%   		&+ f(k_1	\eps, \cdots, k_{m-1} \eps, 0) - f(k_1 \eps, \cdots, k_{m-2} \eps,
%   		0, 0) \\
%   		&+ \cdots \\
%   		&+ f(k_1 \eps, 0, \cdots, 0) \\
%   		 &= \sum_{i=1}^{k_m} w_m(k_1 \eps, \cdots,
%   		k_{m-1} \eps, i \eps)
%   		\\
%   		&+ \sum_{i=1}^{k_{m-1}} w_{m-1}(k_1 \eps, \cdots, k_{m-2} \eps,
%   		i \eps) \\
%   		&+ \cdots \\
%   		&+ \sum_{i=1}^{k_1} w_1(i \eps)
%   		\end{align*}
% \end{enumerate}
% 
% Then $\sup_{w \text{ encodes } f} \norm{w}_m \le (\eps^m \cdot
% (\frac{L}{\eps})^m)^{\frac{1}{m}} = L$ \footnote{$w \in R^d$, where $d =
% (\frac{L}{\eps})^m$}.
% For any $s \in S$, $\norm{s}_{\frac{m}{m-1}} \le (\frac{L}{\eps}
% m)^{\frac{m-1}{m}} \le m \frac{L}{\eps}$. Then we have (taking $p =
% \frac{m}{m-1}$ and $q = m$)
% \begin{equation}
% \mathcal{R}(\mathcal{F}_{\mathcal{W}}) \le m \frac{L}{\eps} \cdot L
% \sqrt{\frac{1}{n(m-1)}} = \frac{L^2}{\eps} \frac{m}{\sqrt{m-1}}
% \frac{1}{\sqrt{n}} \approx \frac{ \sqrt{m} L^2}{\eps} \frac{1}{\sqrt{n}}
% \end{equation}

\subsection{Lower Bound on Rademacher Complexity}
Efficient sampling-based algorithms require the expected Rademacher complexity
$\mathcal{R}_n(\mathcal{F}) = E_{v \sim X^n}[\hat{R}_n(\mathcal{F},v)]$ to be
negligible for $n = poly(m, \frac{1}{\eps})$. We show that this
cannot be true for eithor worst-case or expected Rademacher complexity.
\begin{thm}
Fix $\eps$ and $L$, for any $poly_{\eps, L}(m)$ (i.e., polynomial-in-$m$ sample
complexity), there exists $m_0$ \footnote{$m_0$ is the number of items.} and $v = (v_1, v_2,
\cdots, v_k)$ (where $k = poly_{\eps, L}(m_0)$ and $v_i \in [0, L]$)
such that $\hat{R}_k(v) \gg \eps$.
\end{thm}
\begin{proof}
We first claim that there exists a function $Expo(m)$ \footnote{Basically just a
function that grows exponential in $m$} such that for sufficiently large $m$ there exists
$Expo(m)$ subsets (of $[m]$) $\{S_i\}_{i=1}^{Expo(m)}$, each of size
$\sqrt{m}$, such that $|S_i \cap S_j| \le m^{1/3}$ for $i \neq j$. The
existence is shown using the probabilistic method. If we independently
sample two random subsets $S$ and $S'$ of size $\sqrt{m}$ from $[m]$, then $Pr[|S \cap S'| > m^{1/3}] \le
\frac{ {m \choose \sqrt{m}} {\sqrt{m} \choose m^{1/3}} 
{{m - m^{1/3}} \choose {\sqrt{m} - m ^{1/3}}} 
}
{{m \choose \sqrt{m}}{m \choose \sqrt{m}}}
= \frac{\sqrt{m} (\sqrt{m} - 1) \cdots (\sqrt{m} - m^{1/3} + 1)}{m (m - 1)
\cdots (m - m^{1/3} + 1)} \le (\frac{\sqrt{m}}{m - m ^{1/3}})^{m^{1/3}}
\le (\frac{\sqrt{m}}{0.9 m})^{m^{1/3}}$ \footnote{For sufficiently large m.}.
That means if we take $k$ independent samples, then
\begin{equation}
Pr[\cup_{1 \le i < j \le k} \{ |S_i \cap S_j| > m^{1/3} \}]
\le
\sum_{1 \le i < j \le k} Pr[|S_i \cap S_j| > m^{1/3}]
=
{k \choose 2} (\frac{1.1}{\sqrt{m}})^{m^{1/3}}
\end{equation}

For $Pr[\cup_{i < j} \{ |S_i \cap S_j| > m^{1/3} \}] < 1$, we can let $k$ be
exponential in $m$, and there is still
positive probability that no two subsets overlap too much.

Given the $poly_{\eps, L}(m)$, we can always find a $m_0$ such that
$Expo(m_0) \ge poly_{\eps, L}(m_0)$ as the former functions grows faster
than the latter.
Then for this $m_0$, we can find at least $k = poly_{\eps, L}(m_0)$ subsets
$\{S_i\}_{i=1}^k$ of size $\sqrt{m_0}$ that has little overlap.

Define $v_i (i \in [k])$ as such:
\begin{equation}
v_{i,j} = 
\begin{cases}
L &\mbox{if } j \in S_i \\
0 & \mbox{otherwise}. 
\end{cases}
\end{equation}

Now given a Rademacher vector $\lambda = (\lambda_1, \cdots, \lambda_n)$. We
want to maximize $\sum_{i=1}^n \lambda_i f(v_i)$. We propose the following menu of
size $|\{i \in [k] : \lambda_i = 1\}|$: for each $i$ such that $\lambda_i = 1$,
add to the menu $(l_i, 1 - \eps)$ where
\begin{equation}
l_{i,j} = 
\begin{cases}
\frac{1}{\sqrt{m_0}} &\mbox{if } j \in S_i \\
0 & \mbox{otherwise}. 
\end{cases}
\end{equation}
For type $v_i$, if $\lambda_i = -1$, then no lottery has large overlap with
$v_i$. So the menu can only extract little revenue from $v_i$. If $\lambda_i =
1$, then $v_i$ would choose $l_i$ by the same argument.
\begin{align*}
\sup_{f \in \mathcal{F}} \sum_i \lambda_i f(v_i)
\ge L \cdot |\{i \in [k] : \lambda_i = 1\}|
\end{align*}
\begin{equation}
\frac{1}{k} E_{\lambda}[ \sup_{f \in \mathcal{F}} \sum_{i=1}^k \lambda_i f(v_i)]
\ge
\frac{L}{2.5}  
\end{equation}
\end{proof}

\begin{thm}
Let $X_m$ be the uniform distribution over the $Expo(m)$ types in the above
proof.
Fix $\eps$ and $L$,
then for any $poly_{\eps, L}(m)$, there exists $m_0$ such that (let $k =
poly_{\eps, L}(m_0)$) $E_{v \sim X^k}[\hat{R}_k(v)] \ge L/3$.
\end{thm}
\begin{proof}
Note that each $v_i$ is drawn from $X$ indepedently, so
\begin{equation}
Pr[\exists i \neq j \text{ s.t. } v_i = v_j] \le k^2 Pr[v_i = v_j] \le
\frac{k^2}{Expo(m)} = \frac{poly_{\eps, L}(m)^2}{Expo(m)}
\end{equation}
For sufficiently large $m$, this probability is negligible.
So w.h.p, all samples are distinct.
As long as the samples are distinct, the empirical Rademacher complexity
is larger than $\frac{L}{2.5}$.
\end{proof}
\begin{remark}
This means that the idea of sampling does not work generally.
\end{remark}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pricing"
%%% End: 


==> related.tex <==


\paragraph{Related Work.} 
The foundational result in revenue-maximizing mechanism design  is due to  Myerson \cite{Myerson81}, who characterized the  revenue-maximizing auction for a single item. Many works have since sought various extensions of Myerson's result to settings involving multiple items. One line of work \cite{pricerand,alaeibayesian,alaeibayesian2,CDW12,CDW12b} in the computer science community has pursued algorithmic results when  buyers' value distributions are supported on a finite set which is given explicitly. This culminated in revenue maximizing combinatorial auctions in rather general settings, with runtime polynomial in the support of the given value distributions.  Another line of work \cite{chawla07,chawla10a,chawla10b,DW12,hart-nisan-a} studies approximations to the optimal mechanism when the value distributions satisfy structural properties, such as independence across items or a monotone hazard rate. Our work departs somewhat from both these lines of work, and studies the complexity of mechanism design in the more general ``black-box distribution'' model. Closest to our work is the recent paper by Hart and Nisan \cite{hart-nisan-b}, who study the menu-complexity of optimal auctions for general distributions as we do.

Finally, we note that our results bounding the sample complexity of optimal mechanism design can be thought of as an application of the program suggested by Balcan et al \cite{balcan}, albeit in a different context. Specifically, their framework uses the machinery of sample complexity to reduce \emph{prior-free} optimal mechanism design to an analogue of step 2 of our ``algorithm''. In their context, a random sample of half the players plays the role of our distribution $\D$.









%-----------------------

%The following two papers use our "unit-demand"model.  The first shows that randomized mechanisms may be arbitrarily better than deterministic ones (something that we should point out explicitly in the intro...) , and the second shows that the gap is bounded for produce distributions.

%Also, a bunch of papers by Yang Cai, Constantinos Daskalakis, S. Matthew Weinberg show how to find near optimal auctions in time that is polynomial in the support of the distribution, but when the distribution has large support (e.g. a product distribution over item values) this will take exponential time.  This motivates more specifically our investigation as to whether we can "approximate" a distribution with large support by one with small support.

% %Finally, we turn to revenue in combinatorial auctions in the Bayesian setting. Unlike in single-item auctions, where revenue maximization is well understood and computationally tractable under fairly general conditions, an understanding of revenue-maximizing combinatorial auctions has eluded the mechanism design community until recently. 
% The state of the art, developed in a series of recent works \cite{alaeibayesian,alaeibayesian2,DW12,CDW12,CDW12b}, is a revenue-maximizing combinatorial auction in settings that satisfy several assumptions. %,  including that players' valuation functions are 
% %additive over items, and 
% %distributed independently. 
% We turn a critical eye to one assumption made in those works:
% %two main technical conditions. The first condition assumes that players' valuations are \emph{additive} over items --- i.e., a player $i$'s valuation is summarized by a vector $w_i \in \RR^m$ indexed by items, and his valuation is given by $v_i(S) = \sum_{j \in S} w_{ij}$. Second, 
% The implementation of the mechanism requires as input an \emph{explicit representation} of each player's  valuation distribution --- i.e.~an explicit list, for each player $i$, of valuation functions and associated probabilities. 

% This last  assumption is particularly problematic for at least two reasons. First, an auctioneer rarely has such explicit and complete distributional information in practice, particularly when the space of valuations is multidimensional. Second, the support size of a distribution can be exponential in the natural parameters of the problem ($n$ and $m$), and even exponentially longer than the distribution's natural representation. Consider, for example, a buyer $i$ who values bundles of items additively, yet his value for each item is drawn i.i.d from a distribution supported on two real numbers. A more permissive, and arguably more realistic model, is one in which an auctioneer can \emph{sample} players' valuation distributions through \emph{market research.} We intend to examine the limitations of such an auctioneer.



%Previous works have proposed solutions to the pricing problem under different assumptions and model. \cite{costis1}, \cite{costis2} showed how to reduce revenue maximization to virtual welfare maximization for multiple-bidder setting under the assumption that the valuation distribution is explicity given.

% Though our focus in on the single-bidder problem, the main difficulty stems from the restriction that we only have oracle access to the valuation distribution which has unbounded support size. (Note that \cite{pricerand} showed that the optimal lottery pricing be can computed by simply solving a linear programming when the valuation distribution is explicitly given as input).

% When runtime is not allowed to depend of size of support, one elegant result is due to \cite{seqpost} which gave a 2-approximation for the optimal unit-demand item-pricing problem with independent valuations. \cite{huangcai} also gave a PTAS for the problem proposed by \cite{noam12}. Our positive results also propose algorithms whose runtime is independent of the size of the underlying valuation distribution.

% For our impossibility result, it follows the work of \cite{noam13}.
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pricing"
%%% End: 


==> small.tex <==
\section{The Complexity of Small Menus}
\label{sec:small}

------------- THIS SECTION NEEDS TO BE REVAMPED. I PROPOSE THAT IT SHOULD INCLUDE THEOREMS/PROPS 1.1,1.2,1.3,1.6 -----------------

In this section, we consider the mechanism design problem when  an auctioneer is
looking to design a near-optimal ``small'' menu. This may be for one of two reasons: either the auctioneer has reason to believe that there exists a near optimal menu which happens to be small, or else he is constrained by practical considerations to such menus. Specifically, we consider the \emph{$k$-menu pricing problem}, in which the auctioneer must choose a $k$-menu maximizing expected revenue over a distribution $\D$ of valuations given by a black box. In this section,  our only assumption on $\D$ is that it is supported on $\V = [0,1]^m$.


\subsection{The Sample Complexity of Designing Small Menus}

We begin by examining the sampling complexity of the $k$-menu pricing problem. We apply the ideas of Section \ref{sec:nets} to prove that it suffices to sample $\D$ a small number of times. Specifically, when valuations are bounded,  a random sample of $n=\poly(m,k)$ valuations from $\D$ suffices for identifying a near optimal $k$-menu.% This can be viewed as a sample complexity result for the set of small menus, in that it bounds the number of samples needed for the empirical distribution approximate the revenue of the original distribution $\D$ on every such menu. 

\begin{theorem}\label{thm:sample_small}
When $\V=[0,1]^m$, there is an algorithm for the single-buyer mechanism design problem  in the black box model which makes $n=\poly(m,k, \frac{1}{\eps})$ queries, and outputs a $k$-menu $M$ such that $\Rev(M,\D) \geq \Rev_k(\D) - \eps$.
\end{theorem}
 We note that, when a near-optimal small $k$-menu exists, the above theorem yields an $\epsilon$-approximation algorithm for the pricing problem. However this result is information theoretic, and does not provide an efficient algorithm.  
%
The proof of the above theorem follows by combining the proposition below with Lemma \ref{lem:lottery_to_menu_net2} and Theorem \ref{thm:nets2}.
\begin{proposition}\label{prop:lottery_net}
  For every $\eps > 0$, there is an effective $\epsilon$-net $\L(\epsilon) \sse \Delta_m$ of $\Delta_m$ with respect to $[0,1]^m$. Moreover,  $|\L(\epsilon)| \leq \left(\frac{1}{\epsilon}\right)^{\tilde{O}(m)}$.
\end{proposition}
\begin{proof}
  Let $\L(\epsilon)$ be the set of all lotteries $x \in \Delta_m$ in which each entry $x_i$ is an integer multiple of $\frac{\eps}{m}$. Evidently, each $x_i$ may take on at most $\frac{m}{\eps}$ possible values, so $|\L(\epsilon)| \leq \left(\frac{m}{\eps}\right)^m$.

Consider $x \in \Delta_m$. To complete the proof, it suffices to exhibit $x' \in \Psi$ such that $|v \cdot x - v \cdot x'| \leq \epsilon$ for every $v \in [0,1]^m$. Let $x'$ be the result of rounding down each entry of $x$ to the nearest multiple of $\frac{\epsilon}{m}$. Observe that $|v_i x_i - v_i x'_i| \leq \frac{\eps}{m}$. Therefore $|v \cdot x - v \cdot x'| \leq \eps$, as needed.
\end{proof}



\subsection{The Computational Complexity of Designing Small Menus}
%We now consider the task of a seller looking to design an optimal ``small'' menu. Even in settings in which revenue can grow linearly in the size of a menu (Theorem \ref{thm:menu_complexity}), a seller may be constrained to small menus due to practical considerations. As an example, consider a restauranteur looking to design a new dinner menu. As no customer can be reasonably expected to select from thousands of menu items, the restaurant may place a reasonable bound $k$ on the number of meals on offer. 

----------- CONTINUE HERE ------------

In this section, we examine the computational complexity of the algorithmic task associated with Theorem \ref{thm:sample_small}.
Let $X$ be an explicitly given uniform distribution over $\{v_1, \cdots, v_n\} \sse \V$. We define the optimization problem $MAXREV(X,k)$ as that of computing the revenue maximizing menu of size at most $k$ for a buyer drawn uniformly from $X$. 

\begin{theorem}\label{thm:maxrev_nphard}
$MAXREV(X, k)$ in NP-hard to approximate to within any factor better than $\frac{e}{e-1}$, even for valuations $\V= \set{0,1}^m$.
\end{theorem}
\begin{proof}
Let $n=|X|$. As all valuations are $\{0,1\}$ vectors, each $v_i \in \X$ corresponds to a subset $S_i = \{ i
\in [m] : v_i = 1\}$ of the items $[m]$. 

We begin by observing that there is an optimal $k$-menu which is an item pricing menu. When $k\geq m$ this is clear, as the seller can do no better than pricing every item at $1$. Now assume $k <m$, and let $M = \{(x_1,p_1), \ldots (x_k,p_k)
\}$ be an optimal lottery pricing $k$-menu. Let $X_j \subseteq [n]$ denote
the set of valuations $v_i$ that chooses lottery $(x_j, p_j)$. 
Observe that the
sets $X_1,\ldots,X_k$ are disjoint, and the revenue is $\sum_{j=1}^k
\frac{|X_j|}{n} p_j$.
Moreover, by individual
rationality, 
every $v_i \in X_j$ satisfies $v_i \cdot x_j \geq p_j$. 
In other words, an item drawn at random
from lottery $x_j$ ``hits'' $S_i$ with probability at least $p_j$. 

Now, consider drawing $k$ items $j_1,\ldots,j_k$ independently, 
one from each of the lotteries
$x_1,\ldots,x_k$. 
For $x_1$, in expectation, the number of valuations ``hit'' by $j_1$ is at least
$|X_1| p_1$. 
Therefore, there is a set of $k$ items that collectively hit at least
$\sum_{j=1}^k |X_j| p_j$ valuations. Setting a price of $1$ for each of these
items gathers that much in revenue. 



To show NP-hardness, we reduce from the NP-hard problem max cover, which is known to be hard to approximate by any factor better than $\frac{e}{e-1}$. For convenience, we use the ``hitting set'' formulation of max cover. The input to this problem is a family $\S=\set{S_1,\ldots,S_n}$ of subsets of $[m]$, and an integer $k$, and the outputs is a ``hitting set'' $M \sse [m]$ of size at most $k$ maximizing the number of sets $S \in \S$ with which $M$ has a non-empty intersection.   Given an instance $(\S,k)$ of max cover, we construct an instance $(X,k)$ of $MAXREV$ by letting $X = \set{v_S : S \in \S}$, where $v_S$ denotes the indicator vectof of $S \sse [m]$. It is not hard to see that the revenue of the optimal $k$-lottery equals the number of sets in $\S$ hit by the optimal hitting set of size at most $k$. Since this reduction is approximation preserving, hardness of approximation follows.
\end{proof}

\begin{theorem}
There is a polynomial-time $(1-1/e)$-approximation algorithm for $MAXREV(X, k)$ when $\V\sse \set{0,1}^m$.
\end{theorem}
\begin{proof}
  The reduction from the max cover problem used in the proof of Theorem \ref{thm:maxrev_nphard} is reversible. Therefore, using the $(1-1/e)$ approximation for max cover yields the same guarantee for $MAXREV$.
\end{proof}


\subsubsection{Open Question}

\paragraph{Open Question:} What is the best approximation possible for MAXREV when the valuations $\V \sse [0,1]^n$ are arbitrary yet bounded?

\paragraph{Conjecture:} We conjecture that there is no constant approximation algorithm for MAXREV, even when $k=1$. In other words, we conjecture that it is hard to find the best single lottery for an explicitly given list of unit-demand valuations! We make this conjecture because of an apparent similarity between this problem and the problem of finding a ``maximum satisfying linear subsystem.'' To see this connection, we phrase $MAXREV(X,1)$ slightly differently.

\paragraph{Alternative Formulation of $MAXREV$ for $k=1$:} Given a matrix $V$ with nonnegative entries, where $v_i$ is the i'th row of V, find a probability vector $x$ and real number $p$ maximizing $p | V x \geq p|$, where $| Vx \geq p|$ is short-hand for the number of the satisfied equations in the system $V x \geq p$. Given an appropriate guess for $p$, a moment's thought reveals that this problem reduces to finding a nonnegative and non-zero vector x satisfying as many as possible of the inequalities $V' x \geq 0$, where $V'_{ij} = V_{ij} - p$. This appears closely related to the ``maximum satisfying linear subsystem'' problem, though we have not yet succeeded in proving hardness.

\paragraph{Summary of Progress so Far:} We succeeded in proving that maximizing  $|V x \geq p|$ for a \emph{given} price $p$ is as hard to approximate as independent set. However, this does not rule out constant approximation algorithms for $MAXREV(.,1)$, since the problem may be easy to approximate for some $p'$ which is slightly smaller (within a constant factor) than the optimal price. Moreover, an $O(\log n)$ approximation algorithm for $MAXREV(.,1)$ is relatively straightforward by  a bucketing argument, followed by applying the constant approximation algorithm for MAXREV with $\set{0,1}$-valuations. Other than that, we appear to be somewhat stuck, though reductions from unique games or label cover appear to be promising approaches for showing hardness.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pricing"
%%% End: 

